From Forks to Forceps: A New Framework for Instance Segmentation of Surgical Instruments

Minimally invasive surgeries and related applications demand surgical tool classification and segmentation at the instance level. Surgical tools are similar in appearance and are long, thin, and handled at an angle. The fine-tuning of state-of-the-art (SOTA) instance segmentation models trained on natural images for instrument segmentation has difficulty discriminating instrument classes. Our research demonstrates that while the bounding box and segmentation mask are often accurate, the classification head mis-classifies the class label of the surgical instrument. We present a new neural network framework that adds a classification module as a new stage to existing instance segmentation models. This module specializes in improving the classification of instrument masks generated by the existing model. The module comprises multi-scale mask attention, which attends to the instrument region and masks the distracting background features. We propose training our classifier module using metric learning with arc loss to handle low inter-class variance of surgical instruments. We conduct exhaustive experiments on the benchmark datasets EndoVis2017 and EndoVis2018. We demonstrate that our method outperforms all (more than 18) SOTA methods compared with, and improves the SOTA performance by at least 12 points (20%) on the EndoVis2017 benchmark challenge and generalizes effectively across the datasets.

==> 2211/Images/fig_arch.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{Images/SurgicalSegmentation_Updated.pdf}
	\caption{Architecture of the proposed 3-stage neural network model, named \tss, for the instrument segmentation. Whereas the first two stages are similar to the state of the art, we introduce a third stage, named \msma, specializing in classification. We make several innovations in the design of \msma as described in the main text.}
	\label{fig:arch}
\end{figure*}

==> 2211/Images/fig_qual.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=0.9\linewidth]{Images/QualitativeAnalysis_final_compressed.pdf}
	\caption{Qualitative Analysis for the comparison of instance segmentation: 4 symbols are used to show the results; \cmark~represents the instance labeled correctly, \xmark shows the misclassified instance, and `O' represents missed instance, A letter `A' indicates an ambiguous instance, where it is ambiguous to select the class of the instrument either due to over-segmentation or due to multiple copies of instrument classes at the same region. We show better classification in the cases of sparse class, overlapping instruments, and do not miss instrument instances. Our failure cases include cases where the instance shows the only shaft of the instrument and a significant change in instrument orientation.}
	\label{fig:QualitativeAnalysis}
\end{figure*}

==> 2211/Images/fig_teaser.tex <==
% \begin{figure}[t]
% \centering
% \def\imgwidth{0.12\linewidth}
% \subfigure[GT]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_gt.png}
% }
% \subfigure[\cite{TernausNet}]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_ternausnet.png}
% }
% \subfigure[\cite{gonzalez2020isinet}]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_isinet.png}
% } 
% \subfigure[\cite{MaskRCNN}]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_maskrcnn.png}
% }
% \subfigure[\cite{DetectoRS}]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_d2rs.png}
% }
% \subfigure[Ours]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_ours.png}
% }
% \caption{Instrument segmentation produced by various competitive methods on a sample from the EndoVis2017 dataset~\cite{EndoVis_2017}. Each instrument class is shown in a different color. Note that ISINet~\cite{gonzalez2020isinet} gets the segmentation right but classifies incorrectly. We identify instrument misclassification as the primary reason for low performance of the \sota techniques, and propose various architecture modification for accurate classification.}
% \label{fig:Teaser}
% \end{figure}

\begin{figure}[t]
\centering
\def\imgwidth{0.3\linewidth}
\subfigure[GT]{
	\includegraphics[width=\imgwidth]{Images/teaser_gt.png}
}
\subfigure[\cite{TernausNet}]{
	\includegraphics[width=\imgwidth]{Images/teaser_ternausnet.png}
}
\subfigure[\cite{MaskRCNN}]{
	\includegraphics[width=\imgwidth]{Images/teaser_maskrcnn.png}
}
\subfigure[\cite{gonzalez2020isinet}]{
	\includegraphics[width=\imgwidth]{Images/teaser_isinet.png}
} 
\subfigure[\cite{DetectoRS}]{
	\includegraphics[width=\imgwidth]{Images/teaser_d2rs.png}
} 
\subfigure[Ours]{
	\includegraphics[width=\imgwidth]{Images/teaser_ours.png}
}
\caption{Instrument segmentation produced by various competitive methods on a sample from the \evda dataset~\cite{EndoVis_2017}. Each instrument class is shown in a different color. Note that ISINet~\cite{gonzalez2020isinet} gets the segmentation right but classifies incorrectly. We identify instrument misclassification as the primary reason for low performance of the \sota techniques, and propose various architecture modification for accurate classification. To illustrate the severity of the problem, substituting the predicted class label of a MaskRCNN object with the ground truth label improved the model's AP50 score from 0.65 to 0.90.}
\label{fig:Teaser}
\end{figure}
%

% \begin{figure}[t]
% \centering
% \def\imgwidth{0.3\linewidth}
% \subfigure[GT]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_gt.png}
% }
% \subfigure[TernausNet]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_ternausnet.png}
% }
% \subfigure[MaskRCNN]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_maskrcnn.png}
% }
% \subfigure[ISINet]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_isinet.png}
% } 
% \subfigure[DetectoRS]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_d2rs.png}
% } 
% \subfigure[Ours]{
% 	\includegraphics[width=\imgwidth]{Images/teaser_ours.png}
% }
% \caption{Instrument segmentation produced by various competitive methods on a sample from the EndoVis2017 dataset~\cite{EndoVis_2017}. Each instrument class is shown in a different color. Note that ISINet~\cite{gonzalez2020isinet} gets the segmentation right but classifies incorrectly. We identify instrument misclassification as the primary reason for low performance of the \sota techniques, and propose various architecture modification for accurate classification. To indicate the severity of the problem, we observe that just changing the predicted class label of an object predicted by MaskRCNN with the ground truth label improved the AP50 performance of model from 0.65 to 0.90 on the dataset.}
% \label{fig:Teaser}
% \end{figure}

==> 2211/Tables/tab_ablation.tex <==
% \begin{table}[t]
% \centering
% %\resizebox{0.9\linewidth}{!}{%
% 	\setlength{\tabcolsep}{12pt}
% \begin{tabular}{llll}
% \hline
% \textbf{Model}  & \textbf{Ch\_ \iou}   \\ \hline
% Stage 1 \& 2 & Stage 1 \& 2 &   37.97   \\
% Stage 1 \& 2\_wsr &      53.30    \\
% Stage 1 \& 2\_maskc &    57.35    \\
% Stage 1 \& 2\_wma &     57.09  \\
% Stage 3 & Stage 3\_cel &    63.63   \\
% \tss &  72.54   \\
% \hline \\
% \end{tabular}%
% %}
% \caption{Ablation Studies of the proposed method \tss }
% \label{tab:Ablation}
% \end{table}

\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{llll}
\hline
     & \textbf{Model}  & \textbf{Ch\_ \iou} \\ \hline
Stage 1 \& 2 & Stage 1 \& 2     &    37.97    \\
     & Stage 1 \& 2\_wsr &      53.30           \\
     & Stage 1 \& 2\_maskc &    57.35        \\
     & Stage 1 \& 2\_wma &     57.09 \\
Stage 3 & Stage 3\_cel &    63.63   \\
    & \tss &      72.54 \\
     \hline
\end{tabular}%
}
\caption{Ablation Studies of the proposed \tss on \evda}
\label{tab:Ablation}
\end{table}

% & Stage 3\_msf &     70.22  \\

%& \textbf{ISI\_ \iou}  & \textbf{mc \iou}

==> 2211/Tables/tab_challenge_iou.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|c|}{\sota} & \multicolumn{8}{c|}{Videos: 4-fold validation} &  
\multirow{2}{*}{\makecell[c]{Challenge \\ IoU}} 
\\
\cline{1-11}
Method & Conference & Architecture & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 
\\
\hline
\multicolumn{12}{l}{\textbf{\sota Vision Instance Segmentation Methods}} 
\\ 
\hline
CascadeRCNN \cite{CascadeRCNN} & CVPR18 & ResNet-50-FPN & 
18.23 & 37.68 & 79.49 & 81.95 & 26.49 & 39.43 & 28.89 & 23.52 & 41.96 
\\ 
\hline
HTC \cite{HTC} & CVPR19 & ResNet-50-FPN & 
12.92 & 26.83 & 24.49 & 19.85 & 3.55 & 13.58 & 6.31 & 7.1 & 14.33 
\\ 
\hline
MaskScoring\_RCNN \cite{MaskScoringRCNN} & CVPR19 & ResNet-50-FPN & 
15.36 & 35.23 & 78.02 & 60.59 & 24.11 & 48.46 & 15.39 & 43.09 & 40.03 
\\ 
\hline
SipMask \cite{SipMask} & ECCV20 & ResNet-50-FPN & 
14.65 & 18.28 & 2.53 & 0.44 & 1.26 & 14.17 & 0.11 & 13.24 & 10.93 
\\ 
\hline
SimCal \cite{SimCal} & ECCV20 & ResNet-50-FPN & 
16.8 & 35.68 & 76.26 & 68.88 & 26.29 & 44.38 & 24.95 & 24.46 & 39.71 
\\ 
\hline
CondInst \cite{CondInst} & ECCV20 & ResNet-50-FPN & 
16.17 & 25.74 & 81.81 & 42.54 & 28.64 & 19.02 & 29.75 & 25.83 & 33.68 
\\ 
\hline
\multicolumn{1}{|l|}{BMaskRCNN~\cite{BMaskRCNN}} &
  \multicolumn{1}{l|}{ECCV20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{15.29} &
  \multicolumn{1}{l|}{20.45} &
  \multicolumn{1}{l|}{63.59} &
  \multicolumn{1}{l|}{12.11} &
  \multicolumn{1}{l|}{14.7} &
  \multicolumn{1}{l|}{13.19} &
  \multicolumn{1}{l|}{16.97} &
  \multicolumn{1}{l|}{28.8} &
  \multicolumn{1}{l|}{23.14} \\ \hline
\multicolumn{1}{|l|}{SOLO~\cite{SOLO}} &
  \multicolumn{1}{l|}{NeurIPS20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{18.6} &
  \multicolumn{1}{l|}{42.78} &
  \multicolumn{1}{l|}{72.67} &
  \multicolumn{1}{l|}{47.12} &
  \multicolumn{1}{l|}{7.64} &
  \multicolumn{1}{l|}{44.61} &
  \multicolumn{1}{l|}{10.36} &
  \multicolumn{1}{l|}{43.84} &
  \multicolumn{1}{l|}{34.83} \\ \hline
\multicolumn{1}{|l|}{SCNet~\cite{SCNet}} &
  \multicolumn{1}{l|}{AAAI21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{17.8} &
  \multicolumn{1}{l|}{34.31} &
  \multicolumn{1}{l|}{51.03} &
  \multicolumn{1}{l|}{2.48} &
  \multicolumn{1}{l|}{3.93} &
  \multicolumn{1}{l|}{12.82} &
  \multicolumn{1}{l|}{9.24} &
  \multicolumn{1}{l|}{15.77} &
  \multicolumn{1}{l|}{18.42} \\ \hline
\multicolumn{1}{|l|}{MFTA~\cite{MFTA}} &
  \multicolumn{1}{l|}{CVPR21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{11.07} &
  \multicolumn{1}{l|}{25.74} &
  \multicolumn{1}{l|}{60.24} &
  \multicolumn{1}{l|}{23.98} &
  \multicolumn{1}{l|}{22.87} &
  \multicolumn{1}{l|}{14.44} &
  \multicolumn{1}{l|}{20.69} &
  \multicolumn{1}{l|}{19.34} &
  \multicolumn{1}{l|}{24.79} \\ \hline
\multicolumn{1}{|l|}{DetectoRS~\cite{DetectoRS}} &
  \multicolumn{1}{l|}{CVPR21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{23.66} &
  \multicolumn{1}{l|}{37.09} &
  \multicolumn{1}{l|}{60.61} &
  \multicolumn{1}{l|}{33.05} &
  \multicolumn{1}{l|}{7.57} &
  \multicolumn{1}{l|}{21.9} &
  \multicolumn{1}{l|}{6.98} &
  \multicolumn{1}{l|}{12.11} &
  \multicolumn{1}{l|}{25.37} \\ \hline
\multicolumn{1}{|l|}{Orienmask~\cite{Orienmask}} &
  \multicolumn{1}{l|}{ICCV21} &
  \multicolumn{1}{l|}{Darknet-53} &
  \multicolumn{1}{l|}{13.32} &
  \multicolumn{1}{l|}{11.85} &
  \multicolumn{1}{l|}{46.34} &
  \multicolumn{1}{l|}{21.98} &
  \multicolumn{1}{l|}{11.5} &
  \multicolumn{1}{l|}{19.03} &
  \multicolumn{1}{l|}{35.2} &
  \multicolumn{1}{l|}{14.95} &
  \multicolumn{1}{l|}{21.77} \\ \hline
\multicolumn{1}{|l|}{QueryInst~\cite{QueryInst}} &
  \multicolumn{1}{l|}{ICCV21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{13.69} &
  \multicolumn{1}{l|}{22.03} &
  \multicolumn{1}{l|}{0.27} &
  \multicolumn{1}{l|}{2.08} &
  \multicolumn{1}{l|}{1.488} &
  \multicolumn{1}{l|}{2.31} &
  \multicolumn{1}{l|}{2.79} &
  \multicolumn{1}{l|}{8.58} &
  \multicolumn{1}{l|}{6.65} \\ \hline
\multicolumn{1}{|l|}{FASA~\cite{FASA}} &
  \multicolumn{1}{l|}{ICCV21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{14.84} &
  \multicolumn{1}{l|}{22.64} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{0.9} &
  \multicolumn{1}{l|}{3.28} &
  \multicolumn{1}{l|}{5.12} &
  \multicolumn{1}{l|}{2.03} &
  \multicolumn{1}{l|}{5.86} &
  \multicolumn{1}{l|}{6.91} 
  \\ 
  \hline
\multicolumn{12}{l}{\textbf{\sota EndoVis Methods}} 
\\ 
\hline
\multicolumn{1}{|l|}{TernausNet~\cite{TernausNet}} &
  \multicolumn{1}{l|}{ICMLA18} &
  \multicolumn{1}{l|}{UNet11} &
  \multicolumn{1}{l|}{32.52} &
  \multicolumn{1}{l|}{56.22} &
  \multicolumn{1}{l|}{48.65} &
  \multicolumn{1}{l|}{40.86} &
  \multicolumn{1}{l|}{23.4} &
  \multicolumn{1}{l|}{26.48} &
  \multicolumn{1}{l|}{37.07} &
  \multicolumn{1}{l|}{15.62} &
  \multicolumn{1}{l|}{34.61} \\ \hline
\multicolumn{1}{|l|}{MF\_TAPNet~\cite{MFTAPNet}} &
  \multicolumn{1}{l|}{MICCAI19} &
  \multicolumn{1}{l|}{TAPNet} &
  \multicolumn{1}{l|}{25.2} &
  \multicolumn{1}{l|}{49.0} &
  \multicolumn{1}{l|}{59.87} &
  \multicolumn{1}{l|}{48.4} &
  \multicolumn{1}{l|}{34.45} &
  \multicolumn{1}{l|}{36.57} &
  \multicolumn{1}{l|}{38.46} &
  \multicolumn{1}{l|}{14.95} &
  \multicolumn{1}{l|}{36.62} \\ \hline
\multicolumn{1}{|l|}{MaskRCNN~\cite{MaskRCNN, gonzalez2020isinet}} &
  \multicolumn{1}{l|}{ICCV17} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{22.1} &
  \multicolumn{1}{l|}{33.19} &
  \multicolumn{1}{l|}{83.32} &
  \multicolumn{1}{l|}{67.55} &
  \multicolumn{1}{l|}{41.88} &
  \multicolumn{1}{l|}{43.01} &
  \multicolumn{1}{l|}{32.82} &
  \multicolumn{1}{l|}{29.52} &
  \multicolumn{1}{l|}{44.18} 
  \\ 
  \hline
\multicolumn{1}{|l|}{ISINet~\cite{gonzalez2020isinet}} &
  \multicolumn{1}{l|}{MICCAI20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{23.21} &
  \multicolumn{1}{l|}{36.15} &
  \multicolumn{1}{l|}{85.18} &
  \multicolumn{1}{l|}{84.54} &
  \multicolumn{1}{l|}{55.63} &
  \multicolumn{1}{l|}{56.18} &
  \multicolumn{1}{l|}{59.45} &
  \multicolumn{1}{l|}{32.07} &
  \multicolumn{1}{l|}{53.55} \\ \hline
\multicolumn{1}{|l|}{ISINet\_flow~\cite{gonzalez2020isinet}} &
  \multicolumn{1}{l|}{MICCAI20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{23.17} &
  \multicolumn{1}{l|}{36.08} &
  \multicolumn{1}{l|}{85.18} &
  \multicolumn{1}{l|}{84.27} &
  \multicolumn{1}{l|}{55.43} &
  \multicolumn{1}{l|}{56.18} &
  \multicolumn{1}{l|}{59.17} &
  \multicolumn{1}{l|}{31.93} &
  \multicolumn{1}{l|}{55.62} 
  \\ 
  \hline
S3NET (Ours) &  & ResNet-50-FPN &
  \multicolumn{1}{l|}{\textbf{53.55}} &
  \multicolumn{1}{l|}{\textbf{46.94}} &
  \multicolumn{1}{l|}{\textbf{88.38}} &
  \multicolumn{1}{l|}{\textbf{80.71}} &
  \multicolumn{1}{l|}{\textbf{81.93}} &
  \multicolumn{1}{l|}{\textbf{79.96}} &
  \multicolumn{1}{l|}{\textbf{81.61}} &
  \multicolumn{1}{l|}{\textbf{67.24}} &
  \multicolumn{1}{l|}{\textbf{72.54}} 
  \\
  \hline
\end{tabular}%
}
\end{center}
\caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in EndoVis 2017. \emph{\sota vision instance segmentation methods}, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on EndoVis 2017. \emph{EndoVis Methods} have been specifically proposed for medical instrument segmentation.}
\label{tab:challenge_iou_without_post_processing}
\end{table*}



==> 2211/Tables/tab_challenge_iou_new.tex <==
\begin{table*}[t]
\caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in \evda. 
%	\nli, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on \evda. \evs methods have been specifically proposed for medical instrument segmentation.
}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\setlength{\tabcolsep}{2.5pt}
\centering
\begin{tabular}{|lllcll|}
\hline
\multicolumn{3}{|c|}{\textbf{\sota}} & \multicolumn{3}{c|}{\textbf{Challenge \iou}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Method}} &
  \multicolumn{1}{c|}{\textbf{Conference}} &
  \multicolumn{1}{c|}{\textbf{Architecture}} &
  \multicolumn{1}{c|}{\textbf{\evda}} &
  \multicolumn{1}{c|}{\textbf{\evdb}} &
  \multicolumn{1}{c|}{\textbf{\eets}} 
\\ \hline
\multicolumn{6}{|l|}{\textbf{\sota \nli Methods}} 
\\ \hline
\multicolumn{1}{|l|}{CascadeRCNN {[}10{]}} & \multicolumn{1}{l|}{CVPR18}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{44.88} &  \multicolumn{1}{l|}{37.75} &  51.22\\ \hline
\multicolumn{1}{|l|}{HTC {[}12{]}}         & \multicolumn{1}{l|}{CVPR19}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{42.24} & \multicolumn{1}{l|}{36.05} & 48.96 \\ \hline
\multicolumn{1}{|l|}{CondInst {[}50{]}}    & \multicolumn{1}{l|}{ECCV20}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{54.52} & \multicolumn{1}{l|}{74.16} & 48.7 \\ \hline
\multicolumn{1}{|l|}{QueryInst {[}18{]}}   & \multicolumn{1}{l|}{ICCV21}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{45.55} & \multicolumn{1}{l|}{29.15} & 48.12 \\ \hline
\multicolumn{6}{|l|}{\textbf{\sota \evs Methods}} \\ \hline
\multicolumn{1}{|l|}{TernausNet {[}48{]}}  & \multicolumn{1}{l|}{ICMLA18}  & \multicolumn{1}{l|}{UNet11}        & \multicolumn{1}{c|}{34.61} &   \multicolumn{1}{l|}{46.22}  & 0.39 \\ \hline
\multicolumn{1}{|l|}{MF TAPNet {[}31{]}}   & \multicolumn{1}{l|}{MICCAI19} & \multicolumn{1}{l|}{TAPNet}        & \multicolumn{1}{c|}{36.62} &  \multicolumn{1}{l|}{ 67.87} & 1.58 \\ \hline
\multicolumn{1}{|l|}{ISINet {[}21{]}}      & \multicolumn{1}{l|}{MICCAI20} & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{55.62} & \multicolumn{1}{l|}{73.03} & 51.04 \\ \hline
\multicolumn{1}{|l|}{S3NET (Ours)}         & \multicolumn{1}{c|}{---}         & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{\textbf{72.54}} & \multicolumn{1}{l|}{\textbf{75.81}} & \textbf{53.99} \\ \hline
\end{tabular}%
\label{tab:challenge_iou_with_post_processing}
\end{table*}


% \begin{table*}[t]
% \caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in \evda. 
% %	\nli, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on \evda. \evs methods have been specifically proposed for medical instrument segmentation.
% }
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \setlength{\tabcolsep}{8pt}
% \centering
% \begin{tabular}{|lllcll|}
% \hline
% \multicolumn{3}{|c|}{\textbf{\sota}} & \multicolumn{3}{c|}{\textbf{Challenge \iou}} \\ \hline
% \multicolumn{1}{|c|}{\textbf{Method}} &
%   \multicolumn{1}{c|}{\textbf{Conference}} &
%   \multicolumn{1}{c|}{\textbf{Architecture}} &
%   \multicolumn{1}{c|}{\textbf{\evda}} &
%   \multicolumn{1}{c|}{\textbf{\evdb}} &
%   \multicolumn{1}{c|}{\textbf{\eets}} 
% \\ \hline
% \multicolumn{6}{|l|}{\textbf{\sota \nli Methods}} 
% \\ \hline
% \multicolumn{1}{|l|}{CascadeRCNN {[}10{]}} & \multicolumn{1}{l|}{CVPR18}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{44.88} &  \multicolumn{1}{l|}{37.75} &  51.22\\ \hline
% \multicolumn{1}{|l|}{HTC {[}12{]}}         & \multicolumn{1}{l|}{CVPR19}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{42.24} & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{CondInst {[}50{]}}    & \multicolumn{1}{l|}{ECCV20}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{54.52} & \multicolumn{1}{l|}{74.16} & 48.7 \\ \hline
% \multicolumn{1}{|l|}{DetectoRS {[}41{]}}   & \multicolumn{1}{l|}{CVPR21}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{48.44} & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{QueryInst {[}18{]}}   & \multicolumn{1}{l|}{ICCV21}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{45.55} & \multicolumn{1}{l|}{29.15} & 48.12 \\ \hline
% \multicolumn{6}{|l|}{\textbf{\sota \evs Methods}} \\ \hline
% \multicolumn{1}{|l|}{TernausNet {[}48{]}}  & \multicolumn{1}{l|}{ICMLA18}  & \multicolumn{1}{l|}{UNet11}        & \multicolumn{1}{c|}{34.61} &   \multicolumn{1}{l|}{46.22}  & 0.39 \\ \hline
% \multicolumn{1}{|l|}{MF TAPNet {[}31{]}}   & \multicolumn{1}{l|}{MICCAI19} & \multicolumn{1}{l|}{TAPNet}        & \multicolumn{1}{c|}{36.62} &  \multicolumn{1}{l|}{ 67.87} & 1.58 \\ \hline
% \multicolumn{1}{|l|}{MaskRCNN {[}21,24{]}} & \multicolumn{1}{l|}{ICCV17}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{44.18} & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{ISINet {[}21{]}}      & \multicolumn{1}{l|}{MICCAI20} & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{53.55} & \multicolumn{1}{l|}{72.99} & 51.04 \\ \hline
% \multicolumn{1}{|l|}{ISINet flow {[}21{]}} &
%   \multicolumn{1}{l|}{MICCAI20} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{c|}{55.62} &
%   \multicolumn{1}{l|}{73.03} &
%   \\ \hline
% \multicolumn{1}{|l|}{S3NET (Ours)}         & \multicolumn{1}{c|}{---}         & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{\textbf{72.54}} & \multicolumn{1}{l|}{\textbf{75.81}} & \textbf{53.99} \\ \hline
% \end{tabular}%
% \label{tab:challenge_iou_with_post_processing}
% \end{table*}





% \begin{table*}[t]
% \begin{center}
% \caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in EndoVis 2017. \emph{\sota vision instance segmentation methods}, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on EndoVis 2017. \emph{EndoVis Methods} have been specifically proposed for medical instrument segmentation.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{3}{|c|}{\sota} & \multicolumn{8}{c|}{Videos: 4-fold validation} &  
% \multirow{2}{*}{\makecell[c]{Challenge \\ IoU}} 
% \\
% \cline{1-11}
% Method & Conference & Architecture & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 
% \\
% \hline
% \multicolumn{12}{l}{\textbf{\sota Vision Instance Segmentation Methods}} 
% \\ 
% \hline
% \multicolumn{1}{|l|}{CascadeRCNN~\cite{CascadeRCNN}} &
%   \multicolumn{1}{l|}{CVPR18} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{14.87} &
%   \multicolumn{1}{l|}{22.37} &
%   \multicolumn{1}{l|}{82.96} &
%   \multicolumn{1}{l|}{82.47} &
%   \multicolumn{1}{l|}{36.08} &
%   \multicolumn{1}{l|}{51.86} &
%   \multicolumn{1}{l|}{52.16} &
%   16.25 &
%   44.88 \\ \hline
% \multicolumn{1}{|l|}{HTC~\cite{HTC}} &
%   \multicolumn{1}{l|}{CVPR19} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{12.12} &
%   \multicolumn{1}{l|}{19.74} &
%   \multicolumn{1}{l|}{76.45} &
%   \multicolumn{1}{l|}{83.66} &
%   \multicolumn{1}{l|}{41.02} &
%   \multicolumn{1}{l|}{47.73} &
%   \multicolumn{1}{l|}{40.52} &
%   16.72 &
%   42.24\\
% \hline
% \multicolumn{1}{|l|}{CondInst~\cite{CondInst}} &
%   \multicolumn{1}{l|}{ECCV20} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{24.49} &
%   \multicolumn{1}{l|}{28.67} &
%   \multicolumn{1}{l|}{92.56} &
%   \multicolumn{1}{l|}{86.6} &
%   \multicolumn{1}{l|}{55.84} &
%   \multicolumn{1}{l|}{53.87} &
%   \multicolumn{1}{l|}{59.29} &
%   34.88 & 
%   54.52 \\ \hline
% \multicolumn{1}{|l|}{DetectoRS~\cite{DetectoRS}} &
%   \multicolumn{1}{l|}{CVPR21} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{24.17} &
%   \multicolumn{1}{l|}{26.56} &
%   \multicolumn{1}{l|}{87.76} &
%   \multicolumn{1}{l|}{77.51} &
%   \multicolumn{1}{l|}{44.87} &
%   \multicolumn{1}{l|}{47.53} &
%   \multicolumn{1}{l|}{55.33} &
%   23.77 &
%   48.44 \\ \hline
% \multicolumn{1}{|l|}{QueryInst~\cite{QueryInst}} &
%   \multicolumn{1}{l|}{ICCV21} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{18.75} &
%   \multicolumn{1}{l|}{27.95} &
%   \multicolumn{1}{l|}{80.65} &
%   \multicolumn{1}{l|}{82.41} &
%   \multicolumn{1}{l|}{31.82} &
%   \multicolumn{1}{l|}{47.62} &
%   \multicolumn{1}{l|}{54.77} &
%   20.41 &
%   45.55 \\ 
%   \hline
% \multicolumn{12}{l}{\textbf{ \sota EndoVis Methods}} 
% \\ 
% \hline
% \multicolumn{1}{|l|}{TernausNet~\cite{TernausNet}} &
%   \multicolumn{1}{l|}{ICMLA18} &
%   \multicolumn{1}{l|}{UNet11} &
%   \multicolumn{1}{l|}{32.52} &
%   \multicolumn{1}{l|}{56.22} &
%   \multicolumn{1}{l|}{48.65} &
%   \multicolumn{1}{l|}{40.86} &
%   \multicolumn{1}{l|}{23.4} &
%   \multicolumn{1}{l|}{26.48} &
%   \multicolumn{1}{l|}{37.07} &
%   \multicolumn{1}{l|}{15.62} &
%   \multicolumn{1}{l|}{34.61} \\ \hline
% \multicolumn{1}{|l|}{MF\_TAPNet~\cite{MFTAPNet}} &
%   \multicolumn{1}{l|}{MICCAI19} &
%   \multicolumn{1}{l|}{TAPNet} &
%   \multicolumn{1}{l|}{25.2} &
%   \multicolumn{1}{l|}{49.0} &
%   \multicolumn{1}{l|}{59.87} &
%   \multicolumn{1}{l|}{48.4} &
%   \multicolumn{1}{l|}{34.45} &
%   \multicolumn{1}{l|}{36.57} &
%   \multicolumn{1}{l|}{38.46} &
%   \multicolumn{1}{l|}{14.95} &
%   \multicolumn{1}{l|}{36.62} \\ \hline
% \multicolumn{1}{|l|}{MaskRCNN~\cite{MaskRCNN,gonzalez2020isinet}} &
%   \multicolumn{1}{l|}{ICCV17} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{l|}{22.1} &
%   \multicolumn{1}{l|}{33.19} &
%   \multicolumn{1}{l|}{83.32} &
%   \multicolumn{1}{l|}{67.55} &
%   \multicolumn{1}{l|}{41.88} &
%   \multicolumn{1}{l|}{43.01} &
%   \multicolumn{1}{l|}{32.82} &
%   \multicolumn{1}{l|}{29.52} &
%   \multicolumn{1}{l|}{44.18} 
%   \\ 
%   \hline
% \multicolumn{1}{|l|}{ISINet~\cite{gonzalez2020isinet}} &
%   \multicolumn{1}{l|}{MICCAI20} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{l|}{23.21} &
%   \multicolumn{1}{l|}{36.15} &
%   \multicolumn{1}{l|}{85.18} &
%   \multicolumn{1}{l|}{84.54} &
%   \multicolumn{1}{l|}{55.63} &
%   \multicolumn{1}{l|}{56.18} &
%   \multicolumn{1}{l|}{59.45} &
%   \multicolumn{1}{l|}{32.07} &
%   \multicolumn{1}{l|}{53.55} \\ \hline
% \multicolumn{1}{|l|}{ISINet\_flow~\cite{gonzalez2020isinet}} &
%   \multicolumn{1}{l|}{MICCAI20} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{l|}{23.17} &
%   \multicolumn{1}{l|}{36.08} &
%   \multicolumn{1}{l|}{85.18} &
%   \multicolumn{1}{l|}{84.27} &
%   \multicolumn{1}{l|}{55.43} &
%   \multicolumn{1}{l|}{56.18} &
%   \multicolumn{1}{l|}{59.17} &
%   \multicolumn{1}{l|}{31.93} &
%   \multicolumn{1}{l|}{55.62} 
%   \\ 
%   \hline
% S3NET (Ours) &  & ResNet-50-FPN &
%   \multicolumn{1}{l|}{\textbf{53.55}} &
%   \multicolumn{1}{l|}{\textbf{46.94}} &
%   \multicolumn{1}{l|}{\textbf{88.38}} &
%   \multicolumn{1}{l|}{\textbf{80.71}} &
%   \multicolumn{1}{l|}{\textbf{81.93}} &
%   \multicolumn{1}{l|}{\textbf{79.96}} &
%   \multicolumn{1}{l|}{\textbf{81.61}} &
%   \multicolumn{1}{l|}{\textbf{67.24}} &
%   \multicolumn{1}{l|}{\textbf{72.54}} 
%   \\
%   \hline
% \end{tabular}%
% }
% \end{center}
% \label{tab:challenge_iou_without_post_processing}
% \end{table*}



==> 2211/Tables/tab_challenge_iou_post.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|c|}{\sota} &
\multicolumn{8}{c|}{Videos: 4-fold validation} &
\multirow{2}{*}{\makecell[c]{Challenge \\ IoU}} 
\\ 
\cline{1-11}
%\multicolumn{12}{|c|}{vision-based instance segmentation methods after post-processing} 
%& & & & & & & & & 
%\\ 
%\hline
Method & Conference & Architecture & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 
  \\
  \hline
\multicolumn{1}{|l|}{CascadeRCNN~\cite{CascadeRCNN}} &
  \multicolumn{1}{l|}{CVPR18} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.87} &
  \multicolumn{1}{l|}{22.37} &
  \multicolumn{1}{l|}{82.96} &
  \multicolumn{1}{l|}{82.47} &
  \multicolumn{1}{l|}{36.08} &
  \multicolumn{1}{l|}{51.86} &
  \multicolumn{1}{l|}{52.16} &
  16.25 &
  44.88 \\ \hline
\multicolumn{1}{|l|}{HTC~\cite{HTC}} &
  \multicolumn{1}{l|}{CVPR19} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{12.12} &
  \multicolumn{1}{l|}{19.74} &
  \multicolumn{1}{l|}{76.45} &
  \multicolumn{1}{l|}{83.66} &
  \multicolumn{1}{l|}{41.02} &
  \multicolumn{1}{l|}{47.73} &
  \multicolumn{1}{l|}{40.52} &
  16.72 &
  42.24\\ \hline
\multicolumn{1}{|l|}{MaskScoring\_RCNN~\cite{MaskScoringRCNN}} &
  \multicolumn{1}{l|}{CVPR19} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{18.51} &
  \multicolumn{1}{l|}{24.92} &
  \multicolumn{1}{l|}{80.52} &
  \multicolumn{1}{l|}{82.31} &
  \multicolumn{1}{l|}{29.98} &
  \multicolumn{1}{l|}{52.25} &
  \multicolumn{1}{l|}{48.31} &
  17.38 &
   44.27 \\ \hline
\multicolumn{1}{|l|}{SipMask~\cite{SipMask}} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.78} &
  \multicolumn{1}{l|}{26.51} &
  \multicolumn{1}{l|}{67.60} &
  \multicolumn{1}{l|}{50.55} &
  \multicolumn{1}{l|}{32.17} &
  \multicolumn{1}{l|}{39.67} &
  \multicolumn{1}{l|}{19.28} &
  11.21 & 32.72
   \\ \hline
\multicolumn{1}{|l|}{SimCal~\cite{SimCal}
} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{16.31} &
  \multicolumn{1}{l|}{34.04} &
  \multicolumn{1}{l|}{90.71} &
  \multicolumn{1}{l|}{73.74} &
  \multicolumn{1}{l|}{46.17} &
  \multicolumn{1}{l|}{37.65} &
  \multicolumn{1}{l|}{43.71} &
   15.46 &
   44.72 \\ \hline
\multicolumn{1}{|l|}{CondInst~\cite{CondInst}} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{24.49} &
  \multicolumn{1}{l|}{28.67} &
  \multicolumn{1}{l|}{92.56} &
  \multicolumn{1}{l|}{86.6} &
  \multicolumn{1}{l|}{55.84} &
  \multicolumn{1}{l|}{53.87} &
  \multicolumn{1}{l|}{59.29} &
  34.88 & 
  54.52 \\ \hline
\multicolumn{1}{|l|}{BMaskRCNN~\cite{BMaskRCNN}} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{17.34} &
  \multicolumn{1}{l|}{27.11} &
  \multicolumn{1}{l|}{83.93} &
  \multicolumn{1}{l|}{79.21} &
  \multicolumn{1}{l|}{40.21} &
  \multicolumn{1}{l|}{45.18} &
  \multicolumn{1}{l|}{43.47} &
   15.41 &
  43.98 \\ \hline
\multicolumn{1}{|l|}{SOLO~\cite{SOLO}} &
  \multicolumn{1}{l|}{NeurIPS20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.36} &
  \multicolumn{1}{l|}{15.22} &
  \multicolumn{1}{l|}{81.81} &
  \multicolumn{1}{l|}{79.39} &
  \multicolumn{1}{l|}{21.30} &
  \multicolumn{1}{l|}{31.19} &
  \multicolumn{1}{l|}{38.51} &
   24.93 & 38.34
  \\ \hline
\multicolumn{1}{|l|}{SCNet~\cite{SCNet}} &
  \multicolumn{1}{l|}{AAAI21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{15.96} &
  \multicolumn{1}{l|}{31.63} &
  \multicolumn{1}{l|}{60.55} &
  \multicolumn{1}{l|}{70.62} &
  \multicolumn{1}{l|}{43.42} &
  \multicolumn{1}{l|}{27.53} &
  \multicolumn{1}{l|}{56.05} &
   17.47 & 40.40\\ \hline
\multicolumn{1}{|l|}{MFTA~\cite{MFTA}} &
  \multicolumn{1}{l|}{CVPR21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.39} &
  \multicolumn{1}{l|}{31.14} &
  \multicolumn{1}{l|}{78.95} &
  \multicolumn{1}{l|}{80.39} &
  \multicolumn{1}{l|}{30.84} &
  \multicolumn{1}{l|}{40.15} &
  \multicolumn{1}{l|}{38.71} &
   19.76 &
   41.79 \\ \hline
\multicolumn{1}{|l|}{DetectoRS~\cite{DetectoRS}} &
  \multicolumn{1}{l|}{CVPR21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{24.17} &
  \multicolumn{1}{l|}{26.56} &
  \multicolumn{1}{l|}{87.76} &
  \multicolumn{1}{l|}{77.51} &
  \multicolumn{1}{l|}{44.87} &
  \multicolumn{1}{l|}{47.53} &
  \multicolumn{1}{l|}{55.33} &
   23.77 &
  48.44 \\ \hline
\multicolumn{1}{|l|}{Orienmask~\cite{Orienmask}} &
  \multicolumn{1}{l|}{ICCV21} &
  Darknet-53 &
  \multicolumn{1}{l|}{23.17} &
  \multicolumn{1}{l|}{28.96} &
  \multicolumn{1}{l|}{84.74} &
  \multicolumn{1}{l|}{63.58} &
  \multicolumn{1}{l|}{34.22} &
  \multicolumn{1}{l|}{54.12} &
  \multicolumn{1}{l|}{46.47} &
  31.78 & 45.88 \\ \hline
\multicolumn{1}{|l|}{QueryInst~\cite{QueryInst}} &
  \multicolumn{1}{l|}{ICCV21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{18.75} &
  \multicolumn{1}{l|}{27.95} &
  \multicolumn{1}{l|}{80.65} &
  \multicolumn{1}{l|}{82.41} &
  \multicolumn{1}{l|}{31.82} &
  \multicolumn{1}{l|}{47.62} &
  \multicolumn{1}{l|}{54.77} &
   20.41 &
   45.55 \\ \hline
\multicolumn{1}{|l|}{FASA~\cite{FASA}} &
  \multicolumn{1}{l|}{ICCV21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{9.1} &
  \multicolumn{1}{l|}{19.58} &
  \multicolumn{1}{l|}{71.15} &
  \multicolumn{1}{l|}{63.18} &
  \multicolumn{1}{l|}{20.87} &
  \multicolumn{1}{l|}{34.70} &
  \multicolumn{1}{l|}{29.15} &
  12.28  & 32.50
   \\ 
   \hline
\tss (Ours) & & ResNet-50-FPN &
  \multicolumn{1}{l|}{\textbf{53.55}} &
  \multicolumn{1}{l|}{\textbf{46.94}} &
  \multicolumn{1}{l|}{\textbf{88.38}} &
  \multicolumn{1}{l|}{\textbf{80.71}} &
  \multicolumn{1}{l|}{\textbf{81.93}} &
  \multicolumn{1}{l|}{\textbf{79.96}} &
  \multicolumn{1}{l|}{\textbf{81.61}} &
  \multicolumn{1}{l|}{\textbf{67.24}} &
  \multicolumn{1}{l|}{\textbf{72.54}} 
  \\
  \hline
\end{tabular}%
}
\end{center}
	\caption{In \cref{tab:challenge_iou_without_post_processing} we have compared with \sota methods after fine-tuning them on EndoVis dataset. However, we propose a specific post-processing specially for the instrument segmentation scenario which does a non-maximal suppression across the classes. Such post-processing can be applied to other methods as well, and hence for a fair comparison we have done so. The table shows the results after post-processing. Note that other EndoVis methods already do a similar post-processing along with host of others. Hence their results do not change. Note that, we do not claim novelty/contribution over the suggested post-processing, as it is already implemented in EndoVis methods without formally describing/acknowledging it.}
	\label{tab:challenge_iou_after_post_processing}
\end{table*}

==> 2211/Tables/tab_comparison_CADIS.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllllll}
\hline
\textbf{Dataset} &
  \textbf{Method} &
  \textbf{Conference} &
  \textbf{Arch.} &
  \textbf{Ch\_ \iou} &
  \textbf{APm} &
  \textbf{ISI\_IOU} &
  \multicolumn{10}{l}{\textbf{Instrument Classes IOU}} &
  \textbf{mcIOU} \\ \cline{8-17}
\textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{C} &
  \textbf{CC} &
  \textbf{TF} &
  \textbf{PK} &
  \textbf{PH} &
  \textbf{LI} &
  \textbf{IH} &
  \textbf{SK} &
  \textbf{MM} &
  \textbf{CF} &
  \textbf{} \\ \hline
\multirow{23}{*}{\textbf{\cadis}} &
  \textbf{\nli Methods} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
 & CascadeRCNN                          & CVPR18    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & HTC                                  & CVPR19    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MaskScoring\_RCNN                    & CVPR19    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SipMask                              & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SimCal                               & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & CondInst                             & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & BMaskRCNN                            & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SOLO                                 & NeurIPS20 & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SCNet                                & AAAI21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MFTA                                 & CVPR21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & DetectoRS                            & CVPR21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Orienmask                            & ICCV21    & Dknt53 &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & QueryInst                            & ICCV21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & FASA                                 & ICCV21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Mask2Former                          & CVPR22    & Trfmr     &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-18} 
 & \textbf{\evs Methods} &           &           &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & TernausNet-11                        & ICMLA18   & UNet11    &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MF-TAPNET                            & MICCAI19  & UNet      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MaskRCNN\_d                          & ICCV17    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & ISINET                               & MICCAI20  & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & TraSeTR                              & ICRA22    & Trfmr     &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & S3NET (OURS)                         &           & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}%
}
\caption{Performance of \sota instance segmentation methods on \cadis instrument segmentation dataset. APm represents Mean Average Precision of the mask, i.e., AP0.50:0.95}
\label{tab:comparison_CADIS_instance}
\end{table*}

==> 2211/Tables/tab_comparison_EV17_18.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{lllllllllllll}
			\hline
			\textbf{Method} &
			\textbf{Conference} &
			\textbf{Arch.} &
			\textbf{Ch\_} &
			\textbf{ISI\_} &
			\multicolumn{7}{c}{\textbf{Instrument Classes IOU}} &
			\textbf{mc} \\ 
			\cline{6-12}
			\textbf{} &
			\textbf{} &
			\textbf{} &
			\textbf{\iou} &
			\textbf{\iou} &
			\textbf{BF} &
			\textbf{PF} &
			\textbf{LND} &
			\textbf{VS/ SI} &
			\textbf{GR/ CA} &
			\textbf{MCS} &
			\textbf{UP} &
			\textbf{\iou} \\ 
			\hline
			\multicolumn{13}{c}{\textbf{Dataset \evda}} \\
			\hline
			\multicolumn{3}{l}{\textbf{\nli Methods}}    &       &       &       &       &       &       &       &       &       &       
			\\
			MaskRCNN~\cite{MaskRCNN} &
			ICCV17 & R50 & 45.65 & 41.77 & 27.59 & 33.67 & 43.96 & 17.95 & 0.80 & 4.20 & 8.98 & 19.59 
			\\
			CascadeRCNN~\cite{CascadeRCNN}                           & CVPR18    & R50    & 49.03 & 39.9  & 33.47 & 32.03 & 44.1  & 16.36 & 1.38  & 3.74  & 10.94 & 20.29 \\
			HTC~\cite{HTC}                                   & CVPR19    & R50    & 43.81 & 40.39 & 35.86 & 27.01 & 46.3  & 14.16 & 1.36  & 7.05  & 9.4   & 20.96 \\
			MScoring\_RCNN~\cite{MaskScoringRCNN}                      & CVPR19    & R50    & 47.63 & 44.54 & 37.95 & 38.48 & 49.43 & 13.55 & 2.57  & 3.93  & 9.52  & 25.23 \\
			SimCal~\cite{SimCal}                                & ECCV20    & R50    & 49.56 & 45.71 & 39.44 & 38.01 & 46.74 & 16.52 & 1.9   & 1.98  & 13.11 & 23.78 \\
			CondInst~\cite{CondInst}                               & ECCV20    & R50    & 59.02 & 52.12 & 44.29 & 38.03 & 47.38 & 24.77 & 4.51  & 15.21 & 15.67 & 27.12 \\
			BMaskRCNN~\cite{BMaskRCNN}                              & ECCV20    & R50    & 49.81 & 38.81 & 32.89 & 32.82 & 41.93 & 12.66 & 2.07  & 1.37  & 14.43 & 19.74 \\
			SOLO~\cite{SOLO}                                   & NeurIPS20 & R50    & 35.41 & 33.72 & 22.05 & 23.17 & 41.07 & 7.68  & 0     & 11.29 & 4.6   & 15.79 \\
			SCNet~\cite{SCNet}                                  & AAAI21    & R50    & 48.17 & 46.92 & 43.96 & 29.54 & 48.75 & 22.89 & 1.19  & 4.9   & 14.47 & 25.98 \\
			MFTA~\cite{MFTA}                                  & CVPR21    & R50    & 46.16 & 41.77 & 31.16 & 35.07 & 39.9  & 12.05 & 2.28  & 6.08  & 11.61 & 20.27 \\
			DetectoRS~\cite{DetectoRS}                             & CVPR21    & R50    & 50.93 & 47.38 & 48.54 & 34.36 & 49.72 & 20.33 & 2.04  & 8.92  & 10.58 & 24.93 \\
			Orienmask~\cite{Orienmask}                              & ICCV21    & Dknt53  & 42.09 & 39.27 & 40.42 & 28.78 & 44.48 & 12.11 & 3.91  & 15.18 & 12.32 & 23.22 \\
			QueryInst~\cite{QueryInst}                              & ICCV21    & R50    & 33.59 & 33.06 & 20.87 & 12.37 & 46.75 & 10.48 & 0.52  & 0.39  & 4.58  & 15.32 \\
			FASA~\cite{FASA}                                  & ICCV21    & R50    & 34.38 & 29.67 & 20.13 & 18.81 & 39.12 & 8.34  & 0.68  & 2.17  & 3.46  & 13.24 \\
			Mask2Former~\cite{mask2former}                                  & CVPR22    & Trfmr    & 40.39 & 39.84 & 19.60 & 20.22 & 45.44 & 11.95  & 0.00  & 1.48  & 22.10  & 17.78 \\
			\textbf{\tss (+Mask2former)}           &     & R50     & 53.31 & 51.2 & 49.48 & 29.91 & 70.61 & 32.98  & 19.53  & 18.35  & 49.51  & 38.13 \\ 
			\cline{1-13} 
			\multicolumn{3}{l}{\textbf{\evs Methods}}    &       &       &       &       &       &       &       &       &       &       \\
			TernausNet-11~\cite{TernausNet}                         & ICMLA18   & UNet11 & 35.27 & 12.67 & 13.45 & 12.39 & 20.51 & 5.97  & 1.08  & 1     & 16.76 & 10.17 \\
			MF-TAPNET~\cite{MFTAPNet}                             & MICCAI19  & UNet   & 37.35 & 13.49 & 16.39 & 14.11 & 19.01 & 8.11  & 0.31  & 4.09  & 13.4  & 10.77 \\
			ISINET~\cite{gonzalez2020isinet}                             & MICCAI20  & R50    & 55.62 & 52.2  & 38.7  & 38.5  & 50.09 & 27.43 & 2.01  & 28.72 & 12.56 & 28.96 \\
			TraSeTR~\cite{TraSeTR}                                & ICRA22    & Trfmr  & 60.4  & 65.2  & 45.2  & \textbf{56.7}  & 55.8  & \textbf{38.9}  & 11.4  & 31.3  & 18.2  & 36.79 \\
			\textbf{\tss (+MaskRCNN)}   &           & R50    & \textbf{72.54} & \textbf{71.99} & \textbf{75.08} & 54.32 & \textbf{61.84} & 35.5  & \textbf{27.47} & \textbf{43.23} & \textbf{28.38} & \textbf{46.55} \\ 
			\hline
			\multicolumn{13}{c}{\textbf{Dataset \evdb}} \\
			\hline
			\multicolumn{3}{l}{\textbf{\nli Methods}}    &       &       &       &       &       &       &       &       &       &       \\
			MaskRCNN~\cite{MaskRCNN}                           & ICCV17    & R50    & 69.41 & 67.94 & 72.85 & 43.13 & 0.85  & 32.63 & 0     & 86.16 & 0     & 33.66 \\
			CascadeRCNN~\cite{CascadeRCNN}                           & CVPR18    & R50    & 67.11 & 66.29 & 71.22 & 33.6  & 4.94  & 0     & 0     & 90.61 & 2.62  & 29    \\
			HTC~\cite{HTC}                                    & CVPR19    & R50    & 69.07 & 68.04 & 72.45 & 36.64 & 1.64  & 37.04 & 0     & 88.27 & 1.95  & 34    \\
			MScoring\_RCNN~\cite{MaskScoringRCNN}                      & CVPR19    & R50    & 65.19 & 64.04 & 68.69 & 31.23 & 4.81  & 0     & 0     & 88.23 & 1.75  & 27.82 \\
			SimCal~\cite{SimCal}                                & ECCV20    & R50    & 68.56 & 67.58 & 73.67 & 40.35 & 5.57  & 0     & 0     & 89.84 & 0     & 29.92 \\
			CondInst~\cite{CondInst}                               & ECCV20    & R50    & 72.27 & 71.55 & 77.42 & 37.43 & 7.77  & 43.62 & 0     & 87.8  & 0     & 36.29 \\
			BMaskRCNN~\cite{BMaskRCNN}                             & ECCV20    & R50    & 68.94 & 67.23 & 70.04 & 28.91 & 9.97  & 45.01 & 4.28  & 86.73 & 3.31  & 35.46 \\
			SOLO~\cite{SOLO}                                   & NeurIPS20 & R50    & 65.59 & 64.88 & 69.46 & 23.92 & 2.61  & 36.19 & 0     & 87.97 & 0     & 31.45 \\
			SCNet~\cite{SCNet}                                & AAAI21    & R50    & 71.74 & 70.99 & 78.4  & 47.97 & 5.22  & 29.52 & 0     & 86.69 & 0     & 35.4  \\
			MFTA~\cite{MFTA}                                  & CVPR21    & R50    & 69.2  & 67.97 & 71    & 31.62 & 3.93  & 43.48 & 9.9   & 87.77 & 3.86  & 35.94 \\
			DetectoRS~\cite{DetectoRS}                             & CVPR21    & R50    & 66.69 & 65.06 & 73.94 & 46.85 & 0     & 0     & 0     & 79.92 & 0     & 28.67 \\
			Orienmask~\cite{Orienmask}                              & ICCV21    & Dknt53  & 67.69 & 66.77 & 68.95 & 38.66 & 0     & 31.25 & 0     & 91.21 & 0     & 32.87 \\
			QueryInst~\cite{QueryInst}                             & ICCV21    & R50    & 66.44 & 65.82 & 74.13 & 31.68 & 2.3   & 0     & 0     & 87.28 & 0     & 27.91 \\
			FASA~\cite{FASA}                                   & ICCV21    & R50    & 68.31 & 66.84 & 72.82 & 37.64 & 5.62  & 0     & 0     & 89.02 & 1.03  & 29.45 \\
			Mask2Former~\cite{mask2former}                           & CVPR22    & Trfmr  & 65.47 & 64.69 & 69.35 & 24.13 & 0     & 0     & 0     & 89.96 & 10.29 & 27.67 \\
			\textbf{\tss (+Mask2former)} &           & R50    & 67.78 & 67.06 & 71.18 & 29.77 & 1.59  & 0     & 0     & 90.61 & 10.29 & 29.06 \\
			\cline{1-13} 
			\multicolumn{3}{l}{\textbf{\evs Methods}}    &       &       &       &       &       &       &       &       &       &       \\
			TernausNet-11~\cite{TernausNet}                          & ICMLA18   & UNet11 & 46.22 & 39.87 & 44.2  & 4.67  & 0     & 0     & 0     & 50.44 & 0     & 14.19 \\
			MF-TAPNET~\cite{MFTAPNet}                             & MICCAI19  & UNet   & 67.87 & 39.14 & 69.23 & 6.1   & 11.68 & 14    & 0.91  & 70.24 & 0.57  & 24.68 \\
			ISINET~\cite{gonzalez2020isinet}                                & MICCAI20  & R50    & 73.03 & 70.97 & 73.83 & 48.61 & 30.98 & 37.68 & 0     & 88.16 & 2.16  & 40.21 \\
			TraSeTR~\cite{TraSeTR}             & ICRA22    & Trfmr  & \textbf{76.2}  & \_  & 76.3  & ~\textbf{53.3}  & \textbf{46.5} & 40.6  &\textbf{13.9}  & 86.3  & \textbf{17.5}  & \textbf{47.77} \\
			\textbf{\tss (+MaskRCNN)}    &           & R50    & 75.81 & 74.02 & \textbf{77.22} & 50.87 & 19.83 & \textbf{50.59} & 0     & \textbf{92.12} & 7.44  & 42.58 \\ 
			\hline \\
		\end{tabular}%
	} \\
	\caption{Performance of \sota instance segmentation methods on \evda and \evdb instrument segmentation datasets. (R50 represents ResNet-50-FPN, Trfmr represents Transformer,  BF-Bipolar Forceps, PF-Prograsp Forceps, LND-Large Needle Driver, VS/SI- Vessel Sealer/ Suction Instrument, GR/CA- Grasping Retractor/Clip Applier, MCS-Monopolar Curved Scissors, UP-Ultrasound Probe)}
	\label{tab:comparison_EV17_18}
\end{table*}

==> 2211/Tables/tab_comparison_sota.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{lll}
\hline
     & \textbf{Model}  &  \textbf{APm} \\ \hline
 Two-stage & MaskRCNN~\cite{MaskRCNN}   & 45.7    \\  
& CascadeRCNN~\cite{CascadeRCNN}   & 39.6    \\  
     & MaskScoring\_RCNN~\cite{MaskScoringRCNN}   &  44.1    \\   
     & CondInst~\cite{CondInst} & 49.8           \\
     & BMaskRCNN~\cite{BMaskRCNN}    &    36.8      \\
Few-shot     & MFTA~\cite{MFTA} &  33.3      \\
Query-based    & QueryInst~\cite{QueryInst}   &   38.9      \\
 Two-stage + HTC   & HTC~\cite{HTC} &    45.2     \\
    & SCNet~\cite{SCNet}     &     43.9    \\
    & DetectoRS~\cite{DetectoRS}    & 52.5        \\
Long-tail specific & SimCal~\cite{SimCal}   &      42.3    \\
    & FASA~\cite{FASA}   &     29.7    \\
One-stage    & SOLO~\cite{SOLO} &   37.0       \\
     & Orienmask~\cite{Orienmask} &    43.5      \\
Video-Instance     & SipMask~\cite{SipMask} &  30.2         \\
EndoVis  & \tss (Ours) &  \textbf{58.2}          \\
     \hline
\end{tabular}%
}
\caption{Performance of \sota instance segmentation methods on EndoVis 2017 instrument segmentation dataset. APm represents Mean Average Precision of the mask, i.e., AP0.50:0.95}
\label{tab:comparison_sota}
\end{table}

==> 2211/Tables/tab_isinet_iou.tex <==
\begin{table*}[t]
\caption{Class-wise accuracy comparison with \sota (ISINet) on the metric proposed by them. We observe that our results are better for all classes of \evda including sparse class.}
\centering
\resizebox{\linewidth}{!}{ %
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
	\hline
	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{7}{c|}{Instrument Classes - \evda } & mean \\ \cline{3-9}
	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Vessel & Grasping & Monopolar & Ultrasound & class \\
	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Sealer & Retractor & Curved Scissors & Probe & IoU \\ \hline
	ISINet~\cite{gonzalez2020isinet} & 52.2 & 38.7 & 38.5 &	50.09 &	27.43 &	2.01&	28.72&	12.56&	28.96\\ \hline
	\tss (Ours) & \textbf{71.99} & \textbf{75.08} & \textbf{54.32} & \textbf{61.84} & \textbf{35.50} & \textbf{27.47} & \textbf{43.23} & \textbf{28.38} & \textbf{53.64} \\ \hline
\end{tabular}
}
\\ \vspace{1em}
\resizebox{\linewidth}{!}{ %
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}	
	\hline	
	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{7}{c|}{Instrument Classes- \evdb } & mean \\ \cline{3-9}
	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Monopolar & Ultrasound & Suction & Clip &  class\\
	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Curved Scissors & Probe & Instrument & Applier & IoU \\ \hline
	ISINet~\cite{gonzalez2020isinet} & 70.97 &  73.83 & 48.61 &	30.98 &	88.16 &	2.16&	37.68&	0.00 &	40.21\\ \hline
	\tss (Ours) & \textbf{74.02} & \textbf{77.22} & \textbf{50.87} & 19.83 & \textbf{92.12} & \textbf{7.44} & \textbf{50.59} & 0.00 & \textbf{42.58} \\ \hline
\end{tabular}
}
\\ \vspace{1em} %
\resizebox{\linewidth}{!}{ %
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}	
	\hline	
	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{10}{c|}{Instrument Classes- \eets } & mean \\ \cline{3-12}
	\multicolumn{1}{|c|}{} & ISINet & Suction & Irrigation & Spachula & Scissors & Knife & Navigation & Biopsy1 & Curette & Drill & Tumor &  class\\
	\multicolumn{1}{|c|}{} &IoU  &  &  &   &  &  &   & & & & Biopsy& IoU  \\ \hline
	ISINet~\cite{gonzalez2020isinet}& 46.23  & 77.26	& 35.44	& 1.18	& 0.00	& 3.67	& 41.59	& 14.45	& 23.98 & 4.21 &  7.66 & 20.94	 \\ \hline	
	\tss (Ours) & \textbf{49.19} & 76.36 & 29.95 & \textbf{9.15} & 0.00 & \textbf{7.22} & \textbf{46.44} & \textbf{30.46} & 9.82 & 0.00 & \textbf{44.91} & \textbf{25.43} \\ \hline
\end{tabular}%
}
\label{tab:ISINet_IoU}
\end{table*}

% \begin{table*}[t]
% \caption{Class-wise accuracy comparison our method with the best from \sota (ISINet). We report the results in terms of the metric proposed by ISINet itself, i.e., ISINet \iou, class-wise \iou, and mean class \iou. We observe that our results are better for all classes.}
% \centering
% \resizebox{\linewidth}{!}{ %
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
% 	\hline
% 	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{7}{c|}{Instrument Classes} & mean \\ \cline{3-9}
% 	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Vessel & Grasping & Monopolar & Ultrasound & class \\
% 	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Sealer & Retractor & Curved Scissors & Probe & IoU \\ \hline
% 	ISINet~\cite{gonzalez2020isinet}& 49.57 &	36.93&	37.8&	47.06&	24.96&	2.01&	19.99&	13.9&	26.92 \\ \hline	ISINet\_flow~\cite{gonzalez2020isinet} & 52.2 & 38.7 & 38.5 &	50.09 &	27.43 &	2.01&	28.72&	12.56&	28.96\\ \hline
% 	\tss (Ours) & \textbf{71.99} & \textbf{75.08} & \textbf{54.32} & \textbf{61.84} & \textbf{35.50} & \textbf{27.47} & \textbf{43.23} & \textbf{28.38} & \textbf{53.64} \\ \hline
% \end{tabular}
% }
% \\ \vspace{1em}
% \resizebox{\linewidth}{!}{ %
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}	
% 	\hline	
% 	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Monopolar & Ultrasound & Suction & Clip & mean class\\
% 	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Curved Scissors & Probe & Instrument & Applier & IoU \\ \hline
% 	ISINet~\cite{gonzalez2020isinet}& 71.01 & 73.55 &	48.98&	30.38&  88.17&	 2.23&	37.84&	0.00 &	 40.16 \\ \hline	ISINet\_flow~\cite{gonzalez2020isinet} & 70.97 &  73.83 & 48.61 &	30.98 &	88.16 &	2.16&	37.68&	0.00 &	40.21\\ \hline
% 	\tss (Ours) & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \hline
% \end{tabular}
% }
% \\ \vspace{1em} %
% \resizebox{\linewidth}{!}{ %
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}	
% 	\hline	
% 	\multicolumn{1}{|c|}{} & ISINet & Suction & Irrigation & Spachula & Scissors & Knife & Navigation & Biopsy1 & Curette & Drill & Tumor & mean class\\
% 	\multicolumn{1}{|c|}{} &IoU  &  &  &   &  &  &   & & & & Biopsy& IoU  \\ \hline
% 	ISINet~\cite{gonzalez2020isinet}& 46.23  & 77.26	& 35.44	& 1.18	& 0.00	& 3.67	& 41.59	& 14.45	& 23.98 & 4.21 &  7.66 & 20.94	 \\ \hline	ISINet\_flow~\cite{gonzalez2020isinet} &  &  &  &	 &	 &	&	& & & &	&	\\ \hline
% 	\tss (Ours) & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \hline
% \end{tabular}%
% }
% \label{tab:ISINet_IoU}
% \end{table*}

==> 2211/Tables/tab_miou_CADIS.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
\hline
~\textbf{Instrument} & ~\textbf{UPerNet} & ~\textbf{HRNetV2} & ~\textbf{TraSeTR} & ~\textbf{\tss}  \\
~\textbf{classes}            &  ~\cite{upernet}       &  ~\cite{hrnetv2}      &   ~\cite{TraSeTR}      & ~\textbf{(Ours)} \\ \hline
Cannula            & 50      & 49.5    & 53.1    &        \\
Cap. Cystotome     & 54.5    & 61.7    & 64.4    &        \\
Tissue Forceps     & 74      & 78      & 79.2    &        \\
Primary Knife      & 89.5    & 89.3    & 92.3    &        \\
Ph. Handpiece      & 77.6    & 77.9    & 76.2    &        \\
Lens Injector      & 81      & 82.8    & 87.1    &        \\
I/A Handpiece      & 73.6    & 75.3    & 71.3    &        \\
Secondary Knife    & 68.2    & 79.5    & 82.7    &        \\
Micromanipulator   & 63.6    & 64.4    & 66.3    &        \\
Cap. Forceps       & 23      & 27.2    & 26.1    &        \\ \hline
Total              & 65.5    & 68.6    & 69.9    &        \\ \hline
\end{tabular}%
}
\caption{Segmentation results on \cadis dataset.}
\label{tab:comparison_CADIS_miou}
\end{table}

==> 2211/src_main/P_Abstract.tex <==
\begin{abstract}
%
Minimally invasive surgeries and related applications demand surgical tool classification and segmentation at the instance level. Surgical tools are similar in appearance and are long, thin, and handled at an angle. The fine-tuning of state-of-the-art (\sota) instance segmentation models trained on natural images for instrument segmentation has difficulty discriminating instrument classes. Our research demonstrates that while the bounding box and segmentation mask are often accurate, the classification head misclassifies the class label of the surgical instrument. We present a new neural network framework that adds a classification module as a new stage to existing instance segmentation models. This module specializes in improving the classification of instrument masks generated by the existing model. The module comprises multi-scale mask attention, which attends to the instrument region and masks the distracting background features. We propose training our classifier module using metric learning with \emph{arc loss} to handle low inter-class variance of surgical instruments. We conduct exhaustive experiments on the benchmark datasets EndoVis2017 and EndoVis2018. We demonstrate that our method outperforms all (more than 18) \sota methods compared with, and improves the \sota performance by at least 12 points (20\%) on the EndoVis2017 benchmark challenge and generalizes effectively across the datasets. Project page with source code is available at \url{nets-iitd.github.io/s3net}.

% Minimally invasive surgeries and related applications demand surgical tool classification and segmentation at the instance level. Surgical tools are similar in appearance and are often long, thin, and handled at an angle. The fine-tuning of state-of-the-art (\sota) instance segmentation models trained on natural images for instrument segmentation has difficulty differentiating between instrument classes. Our research demonstrates that while the bounding box and segmentation mask are often accurate, the classification head misclassifies the class label of the surgical instrument. Based on this insight, we present a new neural network framework that adds a classification module as a new stage to existing instance segmentation models. This module specializes in improving the classification of instrument masks generated by the existing model. The module comprises multi-scale mask attention, which attends to the instrument region and masks the distracting background features. We propose training the proposed classifier module using metric learning with \emph{arc loss} to handle low inter-class variance of surgical instruments. We conduct exhaustive experiments on the benchmark datasets EndoVis2017 and EndoVis2018. We demonstrate that our method outperforms all (more than 20) \sota methods compared with and improves the \sota performance by at least 12 points (20 percent) on the EndoVis2017 benchmark challenge and generalizes effectively across the datasets. Project page with source code is available at \href{run:https://nets-iitd.github.io/s3net}{nets-iitd.github.io/s3net}.


% \keywords{Minimally invasive surgery, Instrument type segmentation, Instance segmentation, Neurosurgery, robotic surgery}
% Minimally invasive surgeries and related applications require accurate multi-class classification and instance-level segmentation of surgical instruments.  Current state-of-the-art (\sota) instance segmentation techniques fine-tune contemporary models trained on natural images but manage to give a low accuracy only (Challenge $\iou=0.55$). Our study reveals that for these instance segmentation methods, though the bounding box and segmentation mask are usually good, the classification head performs poorly and misclassifies the type of surgical instrument. Based on this insight, we present a new neural network paradigm that adds a three-stage classification architecture to natural image instance segmentation models for surgical instrument transfer learning.
% (1) The proposed third-stage specializes in the accurate classification of instrument masks generated by the second stage. 
% (2) Surgical instruments are typically long, thin, and used obliquely. Hence, bounding boxes typically contain lots of distracting background clutter. We introduce multi-scale mask attention which attends to the exact instrument region for accurate classification. 
% (3) Surgical instruments are visually very similar to each other, hence cross entropy-based training of classifier is insufficient. We propose training the third stage using metric learning with arc loss to handle low inter class variance. 
% We conduct exhaustive experiments on the benchmark datasets EndoVis2017, EndoVis2018 and CADIS. We demonstrate that our method outperforms all of the methods compared with, improves by at least 12 points (20 percent) over the \sota on the EndoVis2017 benchmark challenge, and generalises effectively across all datasets. Detailed ablation study validates importance of each of the above architectural change.
%
%\keywords{Minimally invasive surgery  \and Instrument type segmentation \and Instance segmentation.\and Neurosurgery \and robotic surgery}
\end{abstract}
%
%




==> 2211/src_main/P_Acknowledgements.tex <==
\mypara{Acknowledgements}
This work was supported by Department of Biotechnology, Ministry of Science and Technology, India (Project No. BT/PR13455/CoE/34/24/2015)

==> 2211/src_main/P_Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}

In this study, we investigated the reasons for the low performance of techniques developed for natural image, on the surgical instrument segmentation tasks. We also showed how carefully designed architectural innovations can successfully mitigate the challenges. We conduct exhaustive experiments on the benchmark robot-assisted surgery datasets EndoVis2017 (\evda), and EndoVis2018 (\evdb). The proposed method generalizes well on all these datasets, outperforms the instance segmentation methods with varying backbones, and achieves at least 12 points (20\%) improvement over the \sota on the benchmark \evda challenge. We conclude that adding a third classification stage improves the results for applications involving fine-grained classification, such as surgical tool segmentation. We hope that our analysis and the innovations to mitigate the challenges specific to surgical instruments will spark similar interest among researchers for the effective application of advancements in natural imaging models to surgical imaging tasks. The proposed framework can be used for downstream applications that depend on tool identification and segmentation. We plan to extend the method to include tracking cues and further improve classification accuracy. 
% 

%We conduct exhaustive experiments on the benchmark datasets EndoVis2017, EndoVis2018 and proposed neurosurgical dataset of real transsphenoidal skull-base surgeries. The proposed method generalizes well on all datasets and achieves at least 17 points (30\%) improvement over the \sota on the benchmark EndoVis2017 challenge.

% Furthermore, our proposed dataset on clinical neurosurgery shall result in future research in this surgical specialty where there is constraint in anatomy, low margin of error and high risk of neurological issues in case of any error during surgery.
 


==> 2211/src_main/P_Experiments_And_Analysis.tex <==
\section{Experiments and Results}

\subsection{Implementation Details}

\myfirstpara{Backbones}
%
% The proposed \msma module can be added to any existing instance segmentation backbone. To validate this, we have used \msma with a CNN-based backbone, MaskRCNN~\cite{MaskRCNN}, and a newer transformer-based backbone, Mask2former~\cite{mask2former} generated masks. The transformer-based backbone is used for validation of third stage and performs poorly than the MaskRCNN backbone. We report most of the results using the basic MaskRCNN backbone. We refer to both the models (based on MaskRCNN or Mask2former) as \tss and explicitly specify the backbone when using transformer architecture.  
%The results are improved from both the \nli methods for instrument segmentation (see ~\cref{tab:comparison_EV17_18}).
The proposed \msma module can be added to any existing instance segmentation method as an additional stage. To validate this, we added \msma on two methods with very different architectures: a CNN-based MaskRCNN~\cite{MaskRCNN} and a newer transformer-based Mask2former~\cite{mask2former}. The latter is used for validation of third stage and performs poorly compared to the former. We report most of the results using the MaskRCNN as the initial stage. We refer to both the models (based on MaskRCNN or Mask2former) as \tss and explicitly specify the architecture type when using the transformer architecture.  
%The results are improved from both the \nli methods for instrument segmentation (see ~\cref{tab:comparison_EV17_18}).

\mypara{Training}
We first train the first two stages using a regression loss, cross-entropy classification loss, and per-pixel segmentation loss.  
We have used an ImageNet pre-trained ResNet-50-FPN model to match the \sota ~\cite{gonzalez2020isinet} architecture and finetuned it for the instrument dataset. We resize each image to a size of $(1333,800)$. Stochastic Gradient Descent with a learning rate of $20^{-2}$ is used to train the two stages simultaneously for 12 epochs.

For stage 3 (\msma), we first use the pre-trained weights of ResNet-50-FPN from the box proposal module and freeze them initially to avoid over-fitting. The classification head of the \msma classifier is first trained using ground truth instance masks for ten epochs using cross-entropy-loss. Then it is trained for 15 epochs using arc loss. After 25 epochs, we unfreeze the weights of ResNet also and train the complete \msma classifier end-to-end for five epochs using arc loss. Finally, only the classification layer is trained using cross-entropy loss. For training the \msma classifier, we have resized each image to $(224,224)$. The ground truth masks were resized to $(56, 56)$ while masking the features to match the feature resolution of the last layer of block 3 in ResNet. 
The mask attended classification head of \msma is trained using Adam optimizer with a learning rate of $10^{-5}$, whereas the end-to-end training of \msma is done using a learning rate of $10^{-7}$.

\mypara{Inference}
During inference, we set the score threshold of 0.0 to accommodate all the classes and select only the top 5 instances because a typical frame contains approximately 3 to 4 instruments in the ground truth. 

% \textcolor{red}{We will publicly release the complete source-code and pre-trained  models post-acceptance, which should cover any inadvertent implementation details missed in the above description. The complete source code is also attached as supplementary material if the reviewers want to replicate the results.}

\input{Tables/tab_comparison_EV17_18}
%\input{./Tables/tab_challenge_iou}
%\input{./Tables/tab_challenge_iou_post}
%\input{Tables/tab_comparison_CADIS}
%\input{Tables/tab_isinet_iou}


\subsection{Analysis}

\myfirstpara{Comparison with \textbf{\sota}}
%
We compare \tss for instrument type segmentation with \evs methods that include semantic segmentation~\cite{TernausNet, MFTAPNet} and instance segmentation approaches~\cite{gonzalez2020isinet, TraSeTR}. For the \nli techniques, we use the source code provided by the authors to train the models for the mentioned datasets and use our inference parameters. We add region-based \nms as mentioned in ~\cref{sec:Our_Proposal} as a post-processing step on the predicted masks of an image and report the \iou scores after post-processing for all the models~(see \cref{tab:comparison_EV17_18}). 
\input{./Images/fig_qual}

For \evda, \tss outperforms all the \nli methods and the other \ evs-based instance segmentation methods. It improves over \isinet~\cite{gonzalez2020isinet} by 30\% Ch\_\iou and 60 \% mc\iou, showing that the mask-based classification using stage 3 improves the results by a considerable margin with only using the spatial information. Even though \trasetr~\cite{TraSeTR} explores transformer-based architecture with mask classification paradigm and also uses the temporal information, \tss outperforms it by a margin of 20\% on Ch\_\iou and 26\% on mc\iou achieving the \sota results. 
For \evdb dataset, \tss outperforms \isinet~\cite{gonzalez2020isinet} by a slight margin of 3.8\% on Ch\-\iou and 5.8\% on mc\iou. In comparison to \trasetr, the results are slightly lesser, which shows that for this dataset, apart from classification, other determining factors like temporal information of the instruments favored a tracking-based method.
%For \cadis dataset, \tss improves over \trasetr with a margin of x\% on m\iou that shows that using Stage 3 for improving classification can be generalized over different datasets~\cref{tab:comparison_CADIS_miou}.

% \textcolor{red}{Compared with SOTA, the performance of this method is not significantly improved in other datasets except EV17. The advantages of this method are not well reflected.} \textcolor{red}{Improvement is not obvious in other datasets except EV17.}
\mypara{Validating Reasons for low accuracy of \sota}
%
% \textcolor{red}{R2In Section 4, Validating Reasons for Low Accuracy of SOTA can be illustrated by adding some charts.}
In \cref{tab:comparison_EV17_18}, we compare \sota instance segmentation on \evs datasets. We have analyzed why the \nli models are less accurate. As noted before, we make three claims about \sota's low segmentation accuracy. First, the present two-stage classification heads are weak and are the bottleneck in accuracy. Second, the instrument's oblique posture and design allow the background to seep into the rectangular boxes, complicating classification. Third, cross entropy-based loss makes learning visually similar instruments harder. We investigated all three claims.

For the first claim, we replace a two-stage model's (MaskRCNN) predicted label with the ground truth label. This simple change increases the mask AP50 score from 0.65 to 0.90, showing classification inaccuracy.

We evaluate Video 1 frames of \evda containing ultrasound probes for the second claim. MaskRCNN predicts 37 ultrasound probe bounding boxes out of 224, with 26 having an \iou of 0.75. 22 of the 26 boxes had an aspect ratio greater than 3, whereas just 4 had an aspect ratio less than 3. Elongated boxes' prediction accuracy was 84\%. MaskRCNN has substantially greater accuracy when the ground truth box firmly hugs the instrument.

For the third claim, we compare the outcomes after training the third stage using cross-entropy loss and arc loss-based metric learning.

%\input{Tables/tab_miou_CADIS}
 
%\input{./Images/fig_tsne}

\subsection{Qualitative Analysis}

The qualitative classification accuracy results are shown in \cref{fig:QualitativeAnalysis}. We show the comparative results of a semantic segmentation method, a typical instance segmentation method, and an \evs method qualitatively. We show better classification in the cases of sparse class and overlapping instruments. Our failure cases include cases where the instance shows only the instrument shaft and a significant change in instrument orientation. Our better performance on the sparse class of Grasping retractor is due to the metric learning-based training loss. Because we devise a mask-attention-based classifier, the network performs well in classifying overlapping regions. We only focused on improving the classification of instance segmentation and not on the temporal context because of the high dependency of the classification accuracy for the next stage of applications. A future direction of this problem can be towards improving the masks and improving the instance labels further based on the temporal information.
% \textcolor{red}{R1:No ablation study to verify the effectiveness of each components.
% R2:The importance of each component of the proposed method is not clearly evaluated. Two main components
% are introduced : a) 3rd stage for classification that uses instance masking, b) arc-loss instead of cross-entropy. An ablation study evaluating the performance gains by introducing each component is missing. More specifically the authors should have compared MaskRCNN (i.e the baseline 2-stage model), the 3-stage model that uses the separate classification stage with cross-entropy loss, the 3-stage model with the arc-loss instead of the cross-entropy.}

\input{./Tables/tab_ablation}

\subsection{Ablation studies}
\label{sec:Ablation studies}

\cref{tab:Ablation} gives the result of various ablation studies performed to understand the importance of various modules in our system. We describe the notation below:

\mypara{Stage 1 \& 2}
%
Here, we report the accuracy obtained by our model after 2nd stage without the post-processing. Since our model uses the MaskRCNN backbone for the first two stages, this is essentially the accuracy of MaskRCNN using our hyper-parameters. 

\mypara{Stage 1 \& 2 \_wsr} 
%
Result of the second stage using our post-processing of non-maximal suppression across classes.
  
\mypara{Stage 1 \& 2 \_maskc} 
%
In the current MaskRCNN, classification and mask prediction are performed in parallel. As per the thesis of this paper, the classification of erroneous boxes is fragile. Hence, in this experiment, we have changed the ordering of the stage 2 predictions. Now the classification is not performed parallel to mask prediction, but after the mask prediction and is done on the mask attended features.

\mypara{Stage 1 \& 2 \_wma} 
%
We have explored whether we can use features of stage 2 for classification instead of training a separate classifier stage. In this experiment, we keep the first two stages as is, but after stage 2, use the mask attended features from stage 2 only. The difference between this and the previous configuration is that in the previous config, the original classifier of MaskRCNN was disabled, but in this one, it remains as is.

\mypara{Stage 3 \_cel} 
%
Here we train S3Net third stage-trained using cross-entropy instead of arc loss. The lower accuracy of this configuration serves to validate one of this paper's key observations, that the instrument's visual similarity makes it difficult to classify, and hence learning representation and classification should be disentangled using metric learning.

% \textcolor{red}{Ideally, such an ablation could be conducted to more than one of the datasets and all
% available metrics should be reported ( APm, mean IOU, challenge IOU). Section 4. p. 8 provides only a
% comparison regarding the choice of arc-loss against using cross-entropy for training the classification stage.
% Here, it is again unclear when or whether arc-loss is substituted by cross-entropy at any stage during training
% (this is closely related to the above comment).}



% For a better understanding of the improved gain by our method over the next best method (ISINet), we compare with the method in terms of class-wise accuracy in \cref{tab:ISINet_IoU}.\textcolor{red}{In the last line of Comparison with SOTA in Section 4, "Our method improves the result for all classes". However, Table2 shows that this is not the case, and makes ambiguities, which should be modified.} Our method significantly improves the results for all classes. \footnote{Due to constraints on the paper length, we show qualitative results corresponding to various methods in the supplementary material.}  
% \textcolor{red}{In Table 3, a comparison of NLI models is provided based on the APm metric. These numbers could be placed in Table 1 results and APm could be reported (alongside IoU and Challenge IoU) for all models of Table
% 1, to enable the reader to clearly parse comparisons to the state-of-the-art.}

%
% \mypara{Validating Reasons for Low Accuracy of \sota}
% %
% In \cref{tab:comparison_sota}, we summarize the performance of \nli on \evda in terms of mask AP denoted as APm, which represents Mean Average Precision of the mask, i.e., AP0.50:0.95. We observe that all the models have much lower accuracy. Our analysis revealed three primary reasons\footnote{(1)weak classification head, (2) oblique pose, and (3) low inter class variance} for the same, which have already been discussion in the introduction section.  
% %and have done detailed analysis for the reasons. As discussed earlier in the paper, we also make three claims regarding the reasons for the low accuracy of \sota on instrument segmentation. First, the classification head of the existing two-stage approaches is weak and is the bottleneck in the accuracy. Second, the oblique pose of the instrument and its shape allows a lot of background to creep in the rectangular boxes and creates problems in the classification. Third, visually similar instruments are difficult to learn through cross entropy-based loss. 
% We have performed various toy experiments to validate all the three reasons. To understand the drop due to weak classification head, we experiment by replacing the predicted label of a two-stage model (MaskRCNN) with the ground truth label. We observe that this improves mask AP50 score from 0.65 to 0.90, thus highlighting the severity of the classification error. To understand the impact of oblique pose of instruments, we analyze frames containing ultrasound probes in video 1 of \evda. Out of 224 instances of the true boxes, MaskRCNN predicts 37 boxes for ultrasound probe, of which 26 has an \iou of 0.75 with the ground truth. We observe that out of these 26 boxes, 22 boxes were of aspect ratio $>$ 3, whereas only 4 of them were from aspect ratio $<$ 3. The accuracy of prediction was higher for the elongated boxes by 84\%. Note that oblique instruments will lead to boxes with a lower aspect ratio, and horizontal/vertical instruments will lead to large aspect ratio boxes. It shows that the MaskRCNN has much higher accuracy when the ground truth box tightly hugs the instrument. To understand the impact of low inter-class variance and less represented instruments, we show an ablation study, where we compare the results after training the third stage with cross-entropy loss and metric learning. Using cross-entropy loss the challenge \iou was 63.63 and with metric learning it increases to 72.54. The lower accuracy of this configuration serves to validate that learning representation and classification should be disentangled using metric learning.



%We investigate the performance of the \sota vision methods for the domain-adaptation into instrument segmentation problem. We investigate our hypothesis of misclassification on aspect ratio, and orientation. We selected ultrasound probe in video 1 which suffers most variation in the angle i.e diagonal to cover a entire square portion of the image to horizontal elongated bounding box. For simplicity, we used a basic MaskRCNN network with overlapping instances removed. Out of the 224 instances of the true bounding boxes, 37 predictions were of same class. We selected the detection boxes which showed at least an \iou of 0.75 with the ground truth box, which was 26. Out of this, 22 boxes were of aspect ratio greater than 3 and only 4 of them were from aspect ratio less than 3. The accuracy of prediction were higher for the elongated boxes by 84\%. This proves our hypothesis that the bounding box aspect ratio plays an important role in misclassification. Another important reason for misclassification is class imbalance. The instrument class of Grasping Retractor is the most sparse class and the classification inaccuracy is evident from ~\cref{tab:ISINet_IoU}. The overlapping nature of the instrument usage and typical long, thin nature of a particular instrument type makes the region proposal to contain background as well as other instrument types and confuses the network on which region to focus. We identify that the existing methods with improved architecture also suffers misclassification like the basic maskrcnn framework. All of these methods outputs multiple masks with different labels for the instruments. We added a post-processing step of keeping only top 5 predictions after non-maximal suppression during testing phase and use minimum prediction threshold, sc\_thr = 0.0 to accommodate low-confidence boxes of some classes. We then keep the highest prediction segments for a particular region of the image and remove overlapping segments with an \iou threshold of 0.75 similar to ISINet~\cite{gonzalez2020isinet}. The results after post processing is shown in~\cref{tab:Challenge_IoU_train} (The pre-processing results are added to supplementary) 
% {\color{green} Reviewer 1 comments 3 addressed here explaining the performance of computer vision baselines}
% \input{Tables/tab_ablation}


% \subsection{Ablation studies}
% \label{sec:Ablation studies}

% \cref{tab:Ablation} gives the result of various ablation studies performed to understand the importance of various modules in our system. We describe the notation below.

% \mypara{Stage 1 \& 2}
% %
% Accuracy obtained by our model after 2nd stage without the post-processing. Since our model uses the MaskRCNN backbone for the first two stages, this is essentially the accuracy of MaskRCNN using our hyper-parameters. 

% \mypara{Stage 1 \& 2 \_wsr} 
% %
% Result of the second stage using our post-processing of non-maximal suppression across classes - this is S3Net without stage 3.
  
% \mypara{Stage 1 \& 2 \_maskc} 
% %
% In the current MaskRCNN, classification and mask prediction are performed in parallel. As per the thesis of this paper, classification on erroneous boxes is fragile. Hence, in this experiment, we have changed the ordering of the stage 2 predictions. Now the classification is not performed parallel to mask prediction, but after the mask prediction and is done on the mask attended features.

% \mypara{Stage 1 \& 2 \_wma} 
% %
% We have explored whether we can use features of stage 2 for classification instead of training a separate classifier stage. In this experiment, we keep the first two stages as is, but after stage 2, use the mask attended features from stage 2 only. The difference between this and the previous configuration is that in the previous config, the original classifier of MaskRCNN was disabled, but in this one, it remains as is.

% \mypara{Stage 3 \_cel} 
% %
% Here we study S3Net with third stage-trained using cross-entropy instead of Arc-loss. The lower accuracy of this configuration serves to validate one of the key observations of this paper, that visual similarity of the instrument makes it difficult to classify, and hence learning representation and classification should be disentangled using metric learning.

% In \cref{tab:comparison_EV17_18}, we summarize the performance of \sota instance segmentation suggested for natural images on \evs datasets. We observe that all the models have much lower accuracy and have done detailed analysis for the reasons. As discussed earlier in the paper, we also make three claims regarding the reasons for the low accuracy of \sota on instrument segmentation. First, the classification head of the existing two-stage approaches is weak and is the bottleneck in the accuracy. Second, the oblique pose of the instrument and its shape allows a lot of background to creep in the rectangular boxes and creates problems in the classification. Third, visually similar instruments are difficult to learn through cross entropy-based loss. We have performed various toy experiments to validate all three claims. 

% For the first claim, as described earlier, we experiment by replacing the predicted label of a two-stage model (MaskRCNN) with the ground truth label. We observe that the simple change improves mask AP50 score from 0.65 to 0.90, thus highlighting the severity of the classification error. 

% For the second claim, we analyze frames containing ultrasound probes in video 1. Out of 224 instances of the true bounding boxes, MaskRCNN predicts 37 boxes for ultrasound probe, of which 26 has an \iou of 0.75 with the ground truth. We observe that out of these 26 boxes, 22 boxes were of aspect ratio greater than 3, whereas only 4 of them were from aspect ratio less than 3. The accuracy of prediction was higher for the elongated boxes by 84\%. Note that oblique instruments will lead to boxes with a lower aspect ratio, and horizontal/vertical instruments will lead to large aspect ratio boxes. It shows that the MaskRCNN has much higher accuracy when the ground truth box tightly hugs the instrument.

% For the third claim, we show an ablation study later, where we compare the results after training the third stage with cross-entropy loss and metric learning.


==> 2211/src_main/P_Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\input{Images/fig_teaser} 

The computer vision community has significantly progressed in designing semantic and instance segmentation algorithms in recent years. One of the reasons for the success is the availability of large  datasets~\cite{russakovsky2015imagenet, COCO_dataset, Imagenet_dataset, cityscapes}. On the other hand, due to the advantages of small incisions and rapid recovery, minimally invasive surgeries (MIS) are increasingly accepted in various surgical specialties~\cite{MIS_benefits_2, MIS_benefits_1}. Automated segmentation of a surgical instrument in MIS is an area of active research with high utility. The surgical instrument segmentation poses various challenges depending on the dataset acquisition source, type of surgery and instruments/ tools involved, image resolution, dataset size, tool statistics, challenging conditions (occlusions, rapid appearance changes, specular reflections, smoke, blur, blood spatter)~\cite{visionreference}. 

Most surgical datasets and algorithms structure instrument segmentation as semantic segmentation, which classifies each pixel as one of the instrument class~\cite{TernausNet, hasan2019u, islam2019real, MFTAPNet, PAANet, DMNet}. Due to disconnected regions and occluded/overlapping instruments, the task of assigning an instance label to the semantic segmentation output is non-trivial. However, obtaining an instance-level mask of the manipulating instruments is essential for most surgical instrument segmentation applications that depend on instrument tracking \cite{du2018articulated, kurmann2017simultaneous, sznitman2014fast, jin2018tool, baby2016neuro}. Hence, we argue for formulating the task as multi-class instance segmentation. 

The research in surgical instrument segmentation is largely driven by the EndoVis2017 dataset~\cite{EndoVis_2017}, which is a robotic instrument dataset containing annotations for different instrument types. The dataset contains seven instruments, all of which have a thin, long, tube-like structure. ISINet \cite{du2018articulated} fine-tunes a MaskRCNN \cite{MaskRCNN} backbone for instance segmentation with a reported Challenge \iou score of 0.55. TraSeTR \cite{TraSeTR} uses a transformer architecture that exploits tracking cues to assist surgical instrument segmentation with a Challenge \iou score of 0.6.

\mypara{Contribution 1}
%
We investigated the reasons for low \iou scores of \sota algorithms on medical instrument segmentation. We found that these methods give a reasonable output for the bounding box and segmentation mask but often misclassify the output box/mask (\cref{fig:Teaser}). We believe that our observation is analogous to the one reported by~\cite{wang2020devil} for natural images. The authors have reported that in the dataset with a long tail, the \sota techniques for object detection in natural images give correct region proposals for less frequent classes but often misclassify them. We posit that due to significant visual differences between natural objects and medical instruments, a deep neural network model that does cross-domain fine-tuning is unable to develop robust features for classification. However, since the bounding box and mask predictions are based on more robust features such as edges, these predictions generalize more easily. Therefore, there is a need for a specialized module in these techniques that focuses on acquiring the attributes necessary for efficiently classifying surgical instruments. Hence, we propose adding a dedicated classification module as a new stage in the existing techniques, which decouples the classification from the bounding box and mask prediction and specializes in classifying classes from the tail of a distribution.

\mypara{Contribution 2}
%
A deeper investigation found a variation in aspect ratio and orientation between natural images and MIS. While in natural images, the width-to-height ratio is usually around 0.5, surgical instruments are mostly two or greater. Further, natural objects appear mostly vertical in an image and fit well in rectilinear bounding boxes. On the other hand, surgical instruments are used obliquely and appear across a bounding box's diagonal. The instrument's aspect ratio and oblique appearance reduce its proportion in the bounding box area and brings in a distracting background.
To make matters worse, given the small operating regions in an MIS, a proposed bounding box may contain multiple tools, further complicating the classification task. The finding motivates the need for classification based on mask-based attention rather than the existing bounding box-based one. Hence, we propose to include mask-based attention in the proposed specialized classification module.

\mypara{Contribution 3}
%
Surgical instruments show inter-class appearance similarity and contain long shafts; the only distinguishing characteristic may be the instruments' tips. Therefore, generic cross entropy-based training of classifiers in contemporary architecture is unsuitable for fine-grained classification of surgical tools. Recent literature suggests that for small datasets, it is beneficial to separate representation learning and classification stages \cite{yao2020adaptive}. The first can be achieved using a contrastive loss, followed by fine-tuning for the classification. We follow a similar approach and train our proposed classification module using arc loss \cite{deng2019arcface}, followed by fine-tuning with cross-entropy loss.

\mypara{Results}
%
We conduct exhaustive experiments on the benchmark Robot-assisted surgery datasets EndoVis2017 (\evda), and EndoVis2018 (\evdb).
%and Cataract Dataset (\cadis). 
The proposed method generalizes well on all these datasets, outperforms the instance segmentation methods with varying backbones, and achieves at least 12 points (20\%) improvement over the \sota on the benchmark EndoVis2017 challenge.
%
% ~\textcolor{red}{We will make the source code and pre-trained models corresponding to this paper publicly available post-publication. The source code has also been uploaded as supplementary material to this submission.}


==> 2211/src_main/P_Our_Proposal.tex <==
\section{Proposed Architecture}
\label{sec:Our_Proposal}

As such, our main contribution, the specialized classification module as a new stage, can be inserted into any existing instance segmentation model. However, we have based our model on the MaskRCNN \cite{MaskRCNN} backbone for validation. The MaskRCNN backbone contains two stages corresponding to the region proposal network (RPN) and a classification head generating masks and labels for each proposal. We insert our classification module as the third stage in the MaskRCNN and replace the labels generated by the second stage with the ones generated by our module. The architecture of our proposed Three Stage Deep Neural Network (\tss) is shown in \cref{fig:arch}. %The proposed model (MaskRCNN backbone with our third stage) can handle various challenges in classifying medical instruments as discussed in \cref{sec:introduction}. 

\mypara{Notation}
%
For a given input frame $I_i$, the first stage, (Box Proposal) extracts $l$ bounding box proposals, where $B_{i,j}$ is the $j^\text{th}$ proposal in the $i^\text{th}$ frame. The second stage (Mask Prediction), predicts the mask $P_{i,j,\hat{c}}$ for each instrument using the bounding box proposals. Here, $\hat{c}$ refers to the class predicted at this stage. 

\mypara{Processing of second stage output}
%
The first stage of MaskRCNN and other similar models is called Region Proposal Network (\rpn) and typically outputs many overlapping regions corresponding to a single object instance in the image. The classification head of the MaskRCNN remains weak even after cross-domain fine-tuning. Hence, many of these overlapping boxes get classified as different classes. A typical non-maximal suppression (\nms) step does not reject overlapping boxes corresponding to different classes. If not addressed, this leads to many false-positive predictions by MaskRCNN and other \sota techniques that we have compared within our experiments. Hence, we modify our implementation's standard \nms step to reject overlapping segments in an image across the classes.

\mypara{Handling misclassification}
%
In a two-stage network, we observe that the proposals generated by the first stage \rpn are inaccurate. However, these proposals get refined by the bounding box regression head in the second stage, leading to higher bounding box and mask accuracy after the second stage. However, the classification is performed on the regions cropped out of inaccurate region proposals from the first stage and remains fragile, which makes classification the bottleneck in the instrument segmentation accuracy. Based upon the insight gained from our analysis, we propose a new deep neural network paradigm that uses the first two stages from a standard instance segmentation method but contains an additional third stage specializing in classification based on the masks. We call the proposed classifier as \emph{Multi-Scale Mask Attended Classifier (\msma)}, which updates/corrects the class predictions from the first two stages. Let $\hat{c}$ denote the class label, and $P_{i,j,\hat{c}}$ denote the mask output corresponding to a region proposal. Then the objective of \msma is to take the original image and mask $P_{i,j,\hat{c}}$ as the input and refine the class label from $\hat{c}$ to a more accurate label $c$. The final mask (with updated class label) is denoted as $P_{i,j,c}$. 
%
As described earlier, the bounding box rectangular regions for a medical instrument contain lots of background and the pixels of other instruments. This is due to the instrument shape and how instruments are typically used in a surgery. This distracts the classification head and leads to errors. Hence, instead of using rectangular region proposals, we introduce spatial mask attention in \msma to emphasize the region belonging to the instrument only. 

%Our third stage specializes in classification, which decouples the classification from the bounding box and mask predicted on region proposals. Due to the characteristic aspect ratio and orientation, a specific instrument type often occupies a very small area in a rectilinear box with other overlapping instruments present in the region proposal. Hence, instead of using rectangular region proposals, we introduce spatial mask attention in the third stage to emphasize the instrument spatial regions. 

During training, we use ground truth masks corresponding to the instance, and while testing, we use the mask predicted by the second stage. This hard-mask attention is performed on multi-scale features of the image. This helps our model focus on the correct instrument spatial region in the image, leading to more accurate classification of the mask generated in the second stage of MaskRCNN. Further, to effectively train with a small dataset, we separate learning feature representation and classification in the proposed third stage. We first perform metric learning with arc loss function, followed by a learning classifier with categorical cross-entropy. Below we describe the proposed \msma module.

\mypara{Multi Scale Mask Attended (\msma) Classifier}
%
Convolutional Feature masking ~\cite{convfeaturemasking} was proposed by Dai et al. to exploit shape information to separate objects from the stuff. We adopt this in an instance segmentation framework to separate instruments from the background/ overlapping instruments and improve the classifier. We explore the decoupling property of the mask and the classification head and use a dedicated neural network with multi-scale mask attention for classification. Our proposed paradigm is shown in \cref{fig:arch}. It takes as input the original RGB image $I_i$ and the predicted masks $P_{i,j,\hat{c}}$ of each instrument instance. A ResNet~\cite{he2016deep} backbone is used to extract multi-scale features from $I_i$. 
%
% The output of blocks two, three, four, and five of ResNet are used to constitute the multi-scale features. The lower spatial dimensional features are upscaled so that each feature is of the same spatial dimension. A $1\times 1$ convolution is applied on each of these features to have the same number of channels. For a particular class $\hat{c}$ instance, its corresponding mask is resized to the spatial dimension of the feature mask.
%
Then, the mask $P_{i,j,\hat{c}}$ is multiplied by each feature to create multi-scale mask-attended features. The masked features are then merged using another $1\times 1$ convolution, creating a single feature map for each instance. Note that if multiple instances of a class are predicted in a frame, then the \msma classifier is run separately for each instance.

%The loss $\mathcal{L}$ is only defined on the k-th instance of the class $c$, and other instance outputs do not contribute to the loss. 
%

We learn an embedding layer over the masked feature map, which outputs an embedding, $E_{i,j}$, for each instrument instance. Each $E_{i,j}$ is then used to classify the instrument present in the mask, giving us a new class label $c$ for the mask. 
%The new class prediction is replaced in the predicted mask $P_{i,j,\hat{c}}$ to obtain the final mask $P_{i,j,c}$. 
For training \msma classifier, we utilize arc loss~\cite{deng2019arcface}, as defined below:
\begin{equation*}
	\mathcal{L} = -\frac{1}{C} \sum_{c=1}^{c=C} \log \frac{e^{\cos(\theta_{c}+m)}}{e^{\cos(\theta_{c}+m)} + \sum_{j=1,j\neq c}^{C} e^{\cos \theta_j}}.
\end{equation*} 
Here $C$ is the number of classes, and $m$ is the angular margin enforced between features of different classes. Further, $\theta_{j}$ is the angle formed between the Embedding feature $E_j$ and the weight vector of the $j^\text{th}$ neuron in the final fully connected layer. The arc loss is adapted from the face recognition domain to the surgical domain where the inter-class variance is low; the arc loss tries to maximize the distance between the features of the classes, thereby increasing the classification accuracy. Unlike categorical cross-entropy loss, which computes the dot product between $E_{i,j}$ and each weight vector, the arc loss only depends on the angle between them. Using arc loss removes the effect of the magnitude of the weight vector for the final decision. Since the magnitude of weight vectors is unbounded, they can easily become biased for a class with more samples. Hence, the arc loss handles class imbalance in the data by removing the dependency over the magnitude of weight vectors. Moreover, the arc loss forms a metric-based angular cluster for each class rather than learning a decision boundary between various classes. This is ensured by the angular margin $m$, resulting in better intra-class compactness and inter-class separability despite data scarcity.
% \textcolor{red}{R1: Why arc loss works for training MSMA classifier is no more illustrated. It is hard for the readers to follow. Try to describe more about how arc loss works for training MSMA classifier.} 


==> 2211/src_main/P_Related_Work.tex <==
\section{Related Work}
\label{sec:Related Work}

The application of object detection, segmentation, and tracking in the field of MIS extends to various surgical branches like gynecology, ophthalmology, and neurosurgery~\cite{bodenstedt2018comparative, zadeh2020surgai, ni2019raunet, qin2020towards}. Researchers have contributed different datasets in this regard as well~\cite{EndoVis, ross2020robust, cadis}. Many techniques have been developed using the Endovis challenge datasets. The instrument segmentation problem has been formulated using both semantic~\cite{TernausNet, hasan2019u, islam2019real, MFTAPNet, PAANet, DMNet}, as well as instance segmentation ~\cite{MaskRCNN_by_Anchor_Opt, gonzalez2020isinet, islam2020ap, Mask_then_classify}. The approach for this segmentation can be supervised, semi-supervised or unsupervised methods. The semi-supervised/unsupervised methods handle the data annotation scarcity in the medical domain and explore domain adaptation of the model to surgical scenario ~\cite{sim2real_sahu, liu2020unsupervised_binary, unsupervised_MICCAI20, unsupervised_MICCAI21}. In this work, we are focusing on the supervised instance segmentation problem. 

\mypara{Semantic Segmentation of Medical Instruments}
% 
TernausNet uses U-Net architecture ~\cite{UNet}, on a pre-trained VGG11 or VGG16 backbone~\cite{TernausNet}. It shows the best performance on binary segmentation but performs poorly on the classification of the instrument type. U-NetPlus uses a modified Encoder-Decoder-based U-Net architecture and data augmentation techniques to improve performance~\cite{hasan2019u}. Some methods explore real-time instrument semantic segmentation~\cite{islam2019real, DMNet}. PAANet aggregate multi-scale attentive features ~\cite{PAANet} and MF-TAPNet integrates flow-based temporal priors to an attention pyramid network~\cite{MFTAPNet}. All the methods discussed above use a single-stage approach for semantic segmentation, which often over segments an instrument to multiple classes (see \cite{TernausNet} in \cref{fig:Teaser}).

\mypara{Instance Segmentation of Medical Instruments}
%
The formulation has been explored in two ways: cross-domain fine-tuning of models pre-trained on natural images~\cite{MaskRCNN, MaskRCNN_by_Anchor_Opt, gonzalez2020isinet, TraSeTR}, and custom-designed models for the task~\cite{islam2020ap, Mask_then_classify}. For the first category, researchers have primarily used MaskRCNN~\cite{MaskRCNN}. Kong et al.~\cite{MaskRCNN_by_Anchor_Opt} adapted MaskRCNN by optimizing the anchor scales for instrument types. ISINet~\cite{gonzalez2020isinet} has used fine-tuned MaskRCNN along with a temporal consistency module to exploit the sequential nature of the data. The improved performance in ISINet is due to the non-maximum suppression of regions across various classes and retaining only the highest predicted class for any instrument instance. Their temporal consistency module improves marginally over their instance selection heuristic. TraSeTR~\cite{TraSeTR} is a transformer-based track-to-segment method that incorporates tracking cues for instance segmentation of instruments. This technique relies on the second stage's classification predictions and adds identity matching and contrastive query learning to address surgical instruments with huge temporal variations. AP-MTL~\cite{islam2020ap} has proposed an Encoder-Decoder architecture for real-time instance segmentation. They have shown improvement over a domain-adapted MaskRCNN. Mask-then-classify~\cite{Mask_then_classify} also used an encoder-decoder network, along with a classifier that uses features from the segmentation stage to classify the pixel-wise instances. The approach uses a single-stage network and is prone to classification errors if there are errors in the masks and vice-versa. 

In this work, we focus on the misclassification challenges of the bounding-box-based instance segmentation methods when fine-tuned for instrument segmentation. We propose adding a novel specialized classification module to mitigate the challenges.


==> Tables/tab_challenge_iou.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|c|}{\sota} & \multicolumn{8}{c|}{Videos: 4-fold validation} &  
\multirow{2}{*}{\makecell[c]{Challenge \\ IoU}} 
\\
\cline{1-11}
Method & Conference & Architecture & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 
\\
\hline
\multicolumn{12}{l}{\textbf{\sota Vision Instance Segmentation Methods}} 
\\ 
\hline
CascadeRCNN \cite{CascadeRCNN} & CVPR18 & ResNet-50-FPN & 
18.23 & 37.68 & 79.49 & 81.95 & 26.49 & 39.43 & 28.89 & 23.52 & 41.96 
\\ 
\hline
HTC \cite{HTC} & CVPR19 & ResNet-50-FPN & 
12.92 & 26.83 & 24.49 & 19.85 & 3.55 & 13.58 & 6.31 & 7.1 & 14.33 
\\ 
\hline
MaskScoring\_RCNN \cite{MaskScoringRCNN} & CVPR19 & ResNet-50-FPN & 
15.36 & 35.23 & 78.02 & 60.59 & 24.11 & 48.46 & 15.39 & 43.09 & 40.03 
\\ 
\hline
SipMask \cite{SipMask} & ECCV20 & ResNet-50-FPN & 
14.65 & 18.28 & 2.53 & 0.44 & 1.26 & 14.17 & 0.11 & 13.24 & 10.93 
\\ 
\hline
SimCal \cite{SimCal} & ECCV20 & ResNet-50-FPN & 
16.8 & 35.68 & 76.26 & 68.88 & 26.29 & 44.38 & 24.95 & 24.46 & 39.71 
\\ 
\hline
CondInst \cite{CondInst} & ECCV20 & ResNet-50-FPN & 
16.17 & 25.74 & 81.81 & 42.54 & 28.64 & 19.02 & 29.75 & 25.83 & 33.68 
\\ 
\hline
\multicolumn{1}{|l|}{BMaskRCNN~\cite{BMaskRCNN}} &
  \multicolumn{1}{l|}{ECCV20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{15.29} &
  \multicolumn{1}{l|}{20.45} &
  \multicolumn{1}{l|}{63.59} &
  \multicolumn{1}{l|}{12.11} &
  \multicolumn{1}{l|}{14.7} &
  \multicolumn{1}{l|}{13.19} &
  \multicolumn{1}{l|}{16.97} &
  \multicolumn{1}{l|}{28.8} &
  \multicolumn{1}{l|}{23.14} \\ \hline
\multicolumn{1}{|l|}{SOLO~\cite{SOLO}} &
  \multicolumn{1}{l|}{NeurIPS20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{18.6} &
  \multicolumn{1}{l|}{42.78} &
  \multicolumn{1}{l|}{72.67} &
  \multicolumn{1}{l|}{47.12} &
  \multicolumn{1}{l|}{7.64} &
  \multicolumn{1}{l|}{44.61} &
  \multicolumn{1}{l|}{10.36} &
  \multicolumn{1}{l|}{43.84} &
  \multicolumn{1}{l|}{34.83} \\ \hline
\multicolumn{1}{|l|}{SCNet~\cite{SCNet}} &
  \multicolumn{1}{l|}{AAAI21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{17.8} &
  \multicolumn{1}{l|}{34.31} &
  \multicolumn{1}{l|}{51.03} &
  \multicolumn{1}{l|}{2.48} &
  \multicolumn{1}{l|}{3.93} &
  \multicolumn{1}{l|}{12.82} &
  \multicolumn{1}{l|}{9.24} &
  \multicolumn{1}{l|}{15.77} &
  \multicolumn{1}{l|}{18.42} \\ \hline
\multicolumn{1}{|l|}{MFTA~\cite{MFTA}} &
  \multicolumn{1}{l|}{CVPR21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{11.07} &
  \multicolumn{1}{l|}{25.74} &
  \multicolumn{1}{l|}{60.24} &
  \multicolumn{1}{l|}{23.98} &
  \multicolumn{1}{l|}{22.87} &
  \multicolumn{1}{l|}{14.44} &
  \multicolumn{1}{l|}{20.69} &
  \multicolumn{1}{l|}{19.34} &
  \multicolumn{1}{l|}{24.79} \\ \hline
\multicolumn{1}{|l|}{DetectoRS~\cite{DetectoRS}} &
  \multicolumn{1}{l|}{CVPR21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{23.66} &
  \multicolumn{1}{l|}{37.09} &
  \multicolumn{1}{l|}{60.61} &
  \multicolumn{1}{l|}{33.05} &
  \multicolumn{1}{l|}{7.57} &
  \multicolumn{1}{l|}{21.9} &
  \multicolumn{1}{l|}{6.98} &
  \multicolumn{1}{l|}{12.11} &
  \multicolumn{1}{l|}{25.37} \\ \hline
\multicolumn{1}{|l|}{Orienmask~\cite{Orienmask}} &
  \multicolumn{1}{l|}{ICCV21} &
  \multicolumn{1}{l|}{Darknet-53} &
  \multicolumn{1}{l|}{13.32} &
  \multicolumn{1}{l|}{11.85} &
  \multicolumn{1}{l|}{46.34} &
  \multicolumn{1}{l|}{21.98} &
  \multicolumn{1}{l|}{11.5} &
  \multicolumn{1}{l|}{19.03} &
  \multicolumn{1}{l|}{35.2} &
  \multicolumn{1}{l|}{14.95} &
  \multicolumn{1}{l|}{21.77} \\ \hline
\multicolumn{1}{|l|}{QueryInst~\cite{QueryInst}} &
  \multicolumn{1}{l|}{ICCV21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{13.69} &
  \multicolumn{1}{l|}{22.03} &
  \multicolumn{1}{l|}{0.27} &
  \multicolumn{1}{l|}{2.08} &
  \multicolumn{1}{l|}{1.488} &
  \multicolumn{1}{l|}{2.31} &
  \multicolumn{1}{l|}{2.79} &
  \multicolumn{1}{l|}{8.58} &
  \multicolumn{1}{l|}{6.65} \\ \hline
\multicolumn{1}{|l|}{FASA~\cite{FASA}} &
  \multicolumn{1}{l|}{ICCV21} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{14.84} &
  \multicolumn{1}{l|}{22.64} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{0.9} &
  \multicolumn{1}{l|}{3.28} &
  \multicolumn{1}{l|}{5.12} &
  \multicolumn{1}{l|}{2.03} &
  \multicolumn{1}{l|}{5.86} &
  \multicolumn{1}{l|}{6.91} 
  \\ 
  \hline
\multicolumn{12}{l}{\textbf{\sota EndoVis Methods}} 
\\ 
\hline
\multicolumn{1}{|l|}{TernausNet~\cite{TernausNet}} &
  \multicolumn{1}{l|}{ICMLA18} &
  \multicolumn{1}{l|}{UNet11} &
  \multicolumn{1}{l|}{32.52} &
  \multicolumn{1}{l|}{56.22} &
  \multicolumn{1}{l|}{48.65} &
  \multicolumn{1}{l|}{40.86} &
  \multicolumn{1}{l|}{23.4} &
  \multicolumn{1}{l|}{26.48} &
  \multicolumn{1}{l|}{37.07} &
  \multicolumn{1}{l|}{15.62} &
  \multicolumn{1}{l|}{34.61} \\ \hline
\multicolumn{1}{|l|}{MF\_TAPNet~\cite{MFTAPNet}} &
  \multicolumn{1}{l|}{MICCAI19} &
  \multicolumn{1}{l|}{TAPNet} &
  \multicolumn{1}{l|}{25.2} &
  \multicolumn{1}{l|}{49.0} &
  \multicolumn{1}{l|}{59.87} &
  \multicolumn{1}{l|}{48.4} &
  \multicolumn{1}{l|}{34.45} &
  \multicolumn{1}{l|}{36.57} &
  \multicolumn{1}{l|}{38.46} &
  \multicolumn{1}{l|}{14.95} &
  \multicolumn{1}{l|}{36.62} \\ \hline
\multicolumn{1}{|l|}{MaskRCNN~\cite{MaskRCNN, gonzalez2020isinet}} &
  \multicolumn{1}{l|}{ICCV17} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{22.1} &
  \multicolumn{1}{l|}{33.19} &
  \multicolumn{1}{l|}{83.32} &
  \multicolumn{1}{l|}{67.55} &
  \multicolumn{1}{l|}{41.88} &
  \multicolumn{1}{l|}{43.01} &
  \multicolumn{1}{l|}{32.82} &
  \multicolumn{1}{l|}{29.52} &
  \multicolumn{1}{l|}{44.18} 
  \\ 
  \hline
\multicolumn{1}{|l|}{ISINet~\cite{gonzalez2020isinet}} &
  \multicolumn{1}{l|}{MICCAI20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{23.21} &
  \multicolumn{1}{l|}{36.15} &
  \multicolumn{1}{l|}{85.18} &
  \multicolumn{1}{l|}{84.54} &
  \multicolumn{1}{l|}{55.63} &
  \multicolumn{1}{l|}{56.18} &
  \multicolumn{1}{l|}{59.45} &
  \multicolumn{1}{l|}{32.07} &
  \multicolumn{1}{l|}{53.55} \\ \hline
\multicolumn{1}{|l|}{ISINet\_flow~\cite{gonzalez2020isinet}} &
  \multicolumn{1}{l|}{MICCAI20} &
  \multicolumn{1}{l|}{ResNet-50-FPN} &
  \multicolumn{1}{l|}{23.17} &
  \multicolumn{1}{l|}{36.08} &
  \multicolumn{1}{l|}{85.18} &
  \multicolumn{1}{l|}{84.27} &
  \multicolumn{1}{l|}{55.43} &
  \multicolumn{1}{l|}{56.18} &
  \multicolumn{1}{l|}{59.17} &
  \multicolumn{1}{l|}{31.93} &
  \multicolumn{1}{l|}{55.62} 
  \\ 
  \hline
S3NET (Ours) &  & ResNet-50-FPN &
  \multicolumn{1}{l|}{\textbf{53.55}} &
  \multicolumn{1}{l|}{\textbf{46.94}} &
  \multicolumn{1}{l|}{\textbf{88.38}} &
  \multicolumn{1}{l|}{\textbf{80.71}} &
  \multicolumn{1}{l|}{\textbf{81.93}} &
  \multicolumn{1}{l|}{\textbf{79.96}} &
  \multicolumn{1}{l|}{\textbf{81.61}} &
  \multicolumn{1}{l|}{\textbf{67.24}} &
  \multicolumn{1}{l|}{\textbf{72.54}} 
  \\
  \hline
\end{tabular}%
}
\end{center}
\caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in EndoVis 2017. \emph{\sota vision instance segmentation methods}, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on EndoVis 2017. \emph{EndoVis Methods} have been specifically proposed for medical instrument segmentation.}
\label{tab:challenge_iou_without_post_processing}
\end{table*}



==> Tables/tab_challenge_iou_new.tex <==
\begin{table*}[t]
\caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in \evda. 
%	\nli, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on \evda. \evs methods have been specifically proposed for medical instrument segmentation.
}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\setlength{\tabcolsep}{2.5pt}
\centering
\begin{tabular}{|lllcll|}
\hline
\multicolumn{3}{|c|}{\textbf{\sota}} & \multicolumn{3}{c|}{\textbf{Challenge \iou}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Method}} &
  \multicolumn{1}{c|}{\textbf{Conference}} &
  \multicolumn{1}{c|}{\textbf{Architecture}} &
  \multicolumn{1}{c|}{\textbf{\evda}} &
  \multicolumn{1}{c|}{\textbf{\evdb}} &
  \multicolumn{1}{c|}{\textbf{\eets}} 
\\ \hline
\multicolumn{6}{|l|}{\textbf{\sota \nli Methods}} 
\\ \hline
\multicolumn{1}{|l|}{CascadeRCNN {[}10{]}} & \multicolumn{1}{l|}{CVPR18}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{44.88} &  \multicolumn{1}{l|}{37.75} &  51.22\\ \hline
\multicolumn{1}{|l|}{HTC {[}12{]}}         & \multicolumn{1}{l|}{CVPR19}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{42.24} & \multicolumn{1}{l|}{36.05} & 48.96 \\ \hline
\multicolumn{1}{|l|}{CondInst {[}50{]}}    & \multicolumn{1}{l|}{ECCV20}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{54.52} & \multicolumn{1}{l|}{74.16} & 48.7 \\ \hline
\multicolumn{1}{|l|}{QueryInst {[}18{]}}   & \multicolumn{1}{l|}{ICCV21}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{45.55} & \multicolumn{1}{l|}{29.15} & 48.12 \\ \hline
\multicolumn{6}{|l|}{\textbf{\sota \evs Methods}} \\ \hline
\multicolumn{1}{|l|}{TernausNet {[}48{]}}  & \multicolumn{1}{l|}{ICMLA18}  & \multicolumn{1}{l|}{UNet11}        & \multicolumn{1}{c|}{34.61} &   \multicolumn{1}{l|}{46.22}  & 0.39 \\ \hline
\multicolumn{1}{|l|}{MF TAPNet {[}31{]}}   & \multicolumn{1}{l|}{MICCAI19} & \multicolumn{1}{l|}{TAPNet}        & \multicolumn{1}{c|}{36.62} &  \multicolumn{1}{l|}{ 67.87} & 1.58 \\ \hline
\multicolumn{1}{|l|}{ISINet {[}21{]}}      & \multicolumn{1}{l|}{MICCAI20} & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{55.62} & \multicolumn{1}{l|}{73.03} & 51.04 \\ \hline
\multicolumn{1}{|l|}{S3NET (Ours)}         & \multicolumn{1}{c|}{---}         & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{\textbf{72.54}} & \multicolumn{1}{l|}{\textbf{75.81}} & \textbf{53.99} \\ \hline
\end{tabular}%
\label{tab:challenge_iou_with_post_processing}
\end{table*}


% \begin{table*}[t]
% \caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in \evda. 
% %	\nli, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on \evda. \evs methods have been specifically proposed for medical instrument segmentation.
% }
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \setlength{\tabcolsep}{8pt}
% \centering
% \begin{tabular}{|lllcll|}
% \hline
% \multicolumn{3}{|c|}{\textbf{\sota}} & \multicolumn{3}{c|}{\textbf{Challenge \iou}} \\ \hline
% \multicolumn{1}{|c|}{\textbf{Method}} &
%   \multicolumn{1}{c|}{\textbf{Conference}} &
%   \multicolumn{1}{c|}{\textbf{Architecture}} &
%   \multicolumn{1}{c|}{\textbf{\evda}} &
%   \multicolumn{1}{c|}{\textbf{\evdb}} &
%   \multicolumn{1}{c|}{\textbf{\eets}} 
% \\ \hline
% \multicolumn{6}{|l|}{\textbf{\sota \nli Methods}} 
% \\ \hline
% \multicolumn{1}{|l|}{CascadeRCNN {[}10{]}} & \multicolumn{1}{l|}{CVPR18}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{44.88} &  \multicolumn{1}{l|}{37.75} &  51.22\\ \hline
% \multicolumn{1}{|l|}{HTC {[}12{]}}         & \multicolumn{1}{l|}{CVPR19}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{42.24} & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{CondInst {[}50{]}}    & \multicolumn{1}{l|}{ECCV20}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{54.52} & \multicolumn{1}{l|}{74.16} & 48.7 \\ \hline
% \multicolumn{1}{|l|}{DetectoRS {[}41{]}}   & \multicolumn{1}{l|}{CVPR21}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{48.44} & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{QueryInst {[}18{]}}   & \multicolumn{1}{l|}{ICCV21}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{45.55} & \multicolumn{1}{l|}{29.15} & 48.12 \\ \hline
% \multicolumn{6}{|l|}{\textbf{\sota \evs Methods}} \\ \hline
% \multicolumn{1}{|l|}{TernausNet {[}48{]}}  & \multicolumn{1}{l|}{ICMLA18}  & \multicolumn{1}{l|}{UNet11}        & \multicolumn{1}{c|}{34.61} &   \multicolumn{1}{l|}{46.22}  & 0.39 \\ \hline
% \multicolumn{1}{|l|}{MF TAPNet {[}31{]}}   & \multicolumn{1}{l|}{MICCAI19} & \multicolumn{1}{l|}{TAPNet}        & \multicolumn{1}{c|}{36.62} &  \multicolumn{1}{l|}{ 67.87} & 1.58 \\ \hline
% \multicolumn{1}{|l|}{MaskRCNN {[}21,24{]}} & \multicolumn{1}{l|}{ICCV17}   & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{44.18} & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{ISINet {[}21{]}}      & \multicolumn{1}{l|}{MICCAI20} & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{53.55} & \multicolumn{1}{l|}{72.99} & 51.04 \\ \hline
% \multicolumn{1}{|l|}{ISINet flow {[}21{]}} &
%   \multicolumn{1}{l|}{MICCAI20} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{c|}{55.62} &
%   \multicolumn{1}{l|}{73.03} &
%   \\ \hline
% \multicolumn{1}{|l|}{S3NET (Ours)}         & \multicolumn{1}{c|}{---}         & \multicolumn{1}{l|}{ResNet-50-FPN} & \multicolumn{1}{c|}{\textbf{72.54}} & \multicolumn{1}{l|}{\textbf{75.81}} & \textbf{53.99} \\ \hline
% \end{tabular}%
% \label{tab:challenge_iou_with_post_processing}
% \end{table*}





% \begin{table*}[t]
% \begin{center}
% \caption{Results for 4-fold validation with train-test split as described in the paper. We report results in terms of challenge \iou metric as suggested in EndoVis 2017. \emph{\sota vision instance segmentation methods}, are general purpose instance segmentation techniques which have appeared in last few years and have reported their results on natural images. For the purpose of comparison we have fine-tuned them on EndoVis 2017. \emph{EndoVis Methods} have been specifically proposed for medical instrument segmentation.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{3}{|c|}{\sota} & \multicolumn{8}{c|}{Videos: 4-fold validation} &  
% \multirow{2}{*}{\makecell[c]{Challenge \\ IoU}} 
% \\
% \cline{1-11}
% Method & Conference & Architecture & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 
% \\
% \hline
% \multicolumn{12}{l}{\textbf{\sota Vision Instance Segmentation Methods}} 
% \\ 
% \hline
% \multicolumn{1}{|l|}{CascadeRCNN~\cite{CascadeRCNN}} &
%   \multicolumn{1}{l|}{CVPR18} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{14.87} &
%   \multicolumn{1}{l|}{22.37} &
%   \multicolumn{1}{l|}{82.96} &
%   \multicolumn{1}{l|}{82.47} &
%   \multicolumn{1}{l|}{36.08} &
%   \multicolumn{1}{l|}{51.86} &
%   \multicolumn{1}{l|}{52.16} &
%   16.25 &
%   44.88 \\ \hline
% \multicolumn{1}{|l|}{HTC~\cite{HTC}} &
%   \multicolumn{1}{l|}{CVPR19} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{12.12} &
%   \multicolumn{1}{l|}{19.74} &
%   \multicolumn{1}{l|}{76.45} &
%   \multicolumn{1}{l|}{83.66} &
%   \multicolumn{1}{l|}{41.02} &
%   \multicolumn{1}{l|}{47.73} &
%   \multicolumn{1}{l|}{40.52} &
%   16.72 &
%   42.24\\
% \hline
% \multicolumn{1}{|l|}{CondInst~\cite{CondInst}} &
%   \multicolumn{1}{l|}{ECCV20} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{24.49} &
%   \multicolumn{1}{l|}{28.67} &
%   \multicolumn{1}{l|}{92.56} &
%   \multicolumn{1}{l|}{86.6} &
%   \multicolumn{1}{l|}{55.84} &
%   \multicolumn{1}{l|}{53.87} &
%   \multicolumn{1}{l|}{59.29} &
%   34.88 & 
%   54.52 \\ \hline
% \multicolumn{1}{|l|}{DetectoRS~\cite{DetectoRS}} &
%   \multicolumn{1}{l|}{CVPR21} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{24.17} &
%   \multicolumn{1}{l|}{26.56} &
%   \multicolumn{1}{l|}{87.76} &
%   \multicolumn{1}{l|}{77.51} &
%   \multicolumn{1}{l|}{44.87} &
%   \multicolumn{1}{l|}{47.53} &
%   \multicolumn{1}{l|}{55.33} &
%   23.77 &
%   48.44 \\ \hline
% \multicolumn{1}{|l|}{QueryInst~\cite{QueryInst}} &
%   \multicolumn{1}{l|}{ICCV21} &
%   ResNet-50-FPN &
%   \multicolumn{1}{l|}{18.75} &
%   \multicolumn{1}{l|}{27.95} &
%   \multicolumn{1}{l|}{80.65} &
%   \multicolumn{1}{l|}{82.41} &
%   \multicolumn{1}{l|}{31.82} &
%   \multicolumn{1}{l|}{47.62} &
%   \multicolumn{1}{l|}{54.77} &
%   20.41 &
%   45.55 \\ 
%   \hline
% \multicolumn{12}{l}{\textbf{ \sota EndoVis Methods}} 
% \\ 
% \hline
% \multicolumn{1}{|l|}{TernausNet~\cite{TernausNet}} &
%   \multicolumn{1}{l|}{ICMLA18} &
%   \multicolumn{1}{l|}{UNet11} &
%   \multicolumn{1}{l|}{32.52} &
%   \multicolumn{1}{l|}{56.22} &
%   \multicolumn{1}{l|}{48.65} &
%   \multicolumn{1}{l|}{40.86} &
%   \multicolumn{1}{l|}{23.4} &
%   \multicolumn{1}{l|}{26.48} &
%   \multicolumn{1}{l|}{37.07} &
%   \multicolumn{1}{l|}{15.62} &
%   \multicolumn{1}{l|}{34.61} \\ \hline
% \multicolumn{1}{|l|}{MF\_TAPNet~\cite{MFTAPNet}} &
%   \multicolumn{1}{l|}{MICCAI19} &
%   \multicolumn{1}{l|}{TAPNet} &
%   \multicolumn{1}{l|}{25.2} &
%   \multicolumn{1}{l|}{49.0} &
%   \multicolumn{1}{l|}{59.87} &
%   \multicolumn{1}{l|}{48.4} &
%   \multicolumn{1}{l|}{34.45} &
%   \multicolumn{1}{l|}{36.57} &
%   \multicolumn{1}{l|}{38.46} &
%   \multicolumn{1}{l|}{14.95} &
%   \multicolumn{1}{l|}{36.62} \\ \hline
% \multicolumn{1}{|l|}{MaskRCNN~\cite{MaskRCNN,gonzalez2020isinet}} &
%   \multicolumn{1}{l|}{ICCV17} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{l|}{22.1} &
%   \multicolumn{1}{l|}{33.19} &
%   \multicolumn{1}{l|}{83.32} &
%   \multicolumn{1}{l|}{67.55} &
%   \multicolumn{1}{l|}{41.88} &
%   \multicolumn{1}{l|}{43.01} &
%   \multicolumn{1}{l|}{32.82} &
%   \multicolumn{1}{l|}{29.52} &
%   \multicolumn{1}{l|}{44.18} 
%   \\ 
%   \hline
% \multicolumn{1}{|l|}{ISINet~\cite{gonzalez2020isinet}} &
%   \multicolumn{1}{l|}{MICCAI20} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{l|}{23.21} &
%   \multicolumn{1}{l|}{36.15} &
%   \multicolumn{1}{l|}{85.18} &
%   \multicolumn{1}{l|}{84.54} &
%   \multicolumn{1}{l|}{55.63} &
%   \multicolumn{1}{l|}{56.18} &
%   \multicolumn{1}{l|}{59.45} &
%   \multicolumn{1}{l|}{32.07} &
%   \multicolumn{1}{l|}{53.55} \\ \hline
% \multicolumn{1}{|l|}{ISINet\_flow~\cite{gonzalez2020isinet}} &
%   \multicolumn{1}{l|}{MICCAI20} &
%   \multicolumn{1}{l|}{ResNet-50-FPN} &
%   \multicolumn{1}{l|}{23.17} &
%   \multicolumn{1}{l|}{36.08} &
%   \multicolumn{1}{l|}{85.18} &
%   \multicolumn{1}{l|}{84.27} &
%   \multicolumn{1}{l|}{55.43} &
%   \multicolumn{1}{l|}{56.18} &
%   \multicolumn{1}{l|}{59.17} &
%   \multicolumn{1}{l|}{31.93} &
%   \multicolumn{1}{l|}{55.62} 
%   \\ 
%   \hline
% S3NET (Ours) &  & ResNet-50-FPN &
%   \multicolumn{1}{l|}{\textbf{53.55}} &
%   \multicolumn{1}{l|}{\textbf{46.94}} &
%   \multicolumn{1}{l|}{\textbf{88.38}} &
%   \multicolumn{1}{l|}{\textbf{80.71}} &
%   \multicolumn{1}{l|}{\textbf{81.93}} &
%   \multicolumn{1}{l|}{\textbf{79.96}} &
%   \multicolumn{1}{l|}{\textbf{81.61}} &
%   \multicolumn{1}{l|}{\textbf{67.24}} &
%   \multicolumn{1}{l|}{\textbf{72.54}} 
%   \\
%   \hline
% \end{tabular}%
% }
% \end{center}
% \label{tab:challenge_iou_without_post_processing}
% \end{table*}



==> Tables/tab_challenge_iou_post.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|c|}{\sota} &
\multicolumn{8}{c|}{Videos: 4-fold validation} &
\multirow{2}{*}{\makecell[c]{Challenge \\ IoU}} 
\\ 
\cline{1-11}
%\multicolumn{12}{|c|}{vision-based instance segmentation methods after post-processing} 
%& & & & & & & & & 
%\\ 
%\hline
Method & Conference & Architecture & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 
  \\
  \hline
\multicolumn{1}{|l|}{CascadeRCNN~\cite{CascadeRCNN}} &
  \multicolumn{1}{l|}{CVPR18} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.87} &
  \multicolumn{1}{l|}{22.37} &
  \multicolumn{1}{l|}{82.96} &
  \multicolumn{1}{l|}{82.47} &
  \multicolumn{1}{l|}{36.08} &
  \multicolumn{1}{l|}{51.86} &
  \multicolumn{1}{l|}{52.16} &
  16.25 &
  44.88 \\ \hline
\multicolumn{1}{|l|}{HTC~\cite{HTC}} &
  \multicolumn{1}{l|}{CVPR19} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{12.12} &
  \multicolumn{1}{l|}{19.74} &
  \multicolumn{1}{l|}{76.45} &
  \multicolumn{1}{l|}{83.66} &
  \multicolumn{1}{l|}{41.02} &
  \multicolumn{1}{l|}{47.73} &
  \multicolumn{1}{l|}{40.52} &
  16.72 &
  42.24\\ \hline
\multicolumn{1}{|l|}{MaskScoring\_RCNN~\cite{MaskScoringRCNN}} &
  \multicolumn{1}{l|}{CVPR19} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{18.51} &
  \multicolumn{1}{l|}{24.92} &
  \multicolumn{1}{l|}{80.52} &
  \multicolumn{1}{l|}{82.31} &
  \multicolumn{1}{l|}{29.98} &
  \multicolumn{1}{l|}{52.25} &
  \multicolumn{1}{l|}{48.31} &
  17.38 &
   44.27 \\ \hline
\multicolumn{1}{|l|}{SipMask~\cite{SipMask}} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.78} &
  \multicolumn{1}{l|}{26.51} &
  \multicolumn{1}{l|}{67.60} &
  \multicolumn{1}{l|}{50.55} &
  \multicolumn{1}{l|}{32.17} &
  \multicolumn{1}{l|}{39.67} &
  \multicolumn{1}{l|}{19.28} &
  11.21 & 32.72
   \\ \hline
\multicolumn{1}{|l|}{SimCal~\cite{SimCal}
} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{16.31} &
  \multicolumn{1}{l|}{34.04} &
  \multicolumn{1}{l|}{90.71} &
  \multicolumn{1}{l|}{73.74} &
  \multicolumn{1}{l|}{46.17} &
  \multicolumn{1}{l|}{37.65} &
  \multicolumn{1}{l|}{43.71} &
   15.46 &
   44.72 \\ \hline
\multicolumn{1}{|l|}{CondInst~\cite{CondInst}} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{24.49} &
  \multicolumn{1}{l|}{28.67} &
  \multicolumn{1}{l|}{92.56} &
  \multicolumn{1}{l|}{86.6} &
  \multicolumn{1}{l|}{55.84} &
  \multicolumn{1}{l|}{53.87} &
  \multicolumn{1}{l|}{59.29} &
  34.88 & 
  54.52 \\ \hline
\multicolumn{1}{|l|}{BMaskRCNN~\cite{BMaskRCNN}} &
  \multicolumn{1}{l|}{ECCV20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{17.34} &
  \multicolumn{1}{l|}{27.11} &
  \multicolumn{1}{l|}{83.93} &
  \multicolumn{1}{l|}{79.21} &
  \multicolumn{1}{l|}{40.21} &
  \multicolumn{1}{l|}{45.18} &
  \multicolumn{1}{l|}{43.47} &
   15.41 &
  43.98 \\ \hline
\multicolumn{1}{|l|}{SOLO~\cite{SOLO}} &
  \multicolumn{1}{l|}{NeurIPS20} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.36} &
  \multicolumn{1}{l|}{15.22} &
  \multicolumn{1}{l|}{81.81} &
  \multicolumn{1}{l|}{79.39} &
  \multicolumn{1}{l|}{21.30} &
  \multicolumn{1}{l|}{31.19} &
  \multicolumn{1}{l|}{38.51} &
   24.93 & 38.34
  \\ \hline
\multicolumn{1}{|l|}{SCNet~\cite{SCNet}} &
  \multicolumn{1}{l|}{AAAI21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{15.96} &
  \multicolumn{1}{l|}{31.63} &
  \multicolumn{1}{l|}{60.55} &
  \multicolumn{1}{l|}{70.62} &
  \multicolumn{1}{l|}{43.42} &
  \multicolumn{1}{l|}{27.53} &
  \multicolumn{1}{l|}{56.05} &
   17.47 & 40.40\\ \hline
\multicolumn{1}{|l|}{MFTA~\cite{MFTA}} &
  \multicolumn{1}{l|}{CVPR21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{14.39} &
  \multicolumn{1}{l|}{31.14} &
  \multicolumn{1}{l|}{78.95} &
  \multicolumn{1}{l|}{80.39} &
  \multicolumn{1}{l|}{30.84} &
  \multicolumn{1}{l|}{40.15} &
  \multicolumn{1}{l|}{38.71} &
   19.76 &
   41.79 \\ \hline
\multicolumn{1}{|l|}{DetectoRS~\cite{DetectoRS}} &
  \multicolumn{1}{l|}{CVPR21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{24.17} &
  \multicolumn{1}{l|}{26.56} &
  \multicolumn{1}{l|}{87.76} &
  \multicolumn{1}{l|}{77.51} &
  \multicolumn{1}{l|}{44.87} &
  \multicolumn{1}{l|}{47.53} &
  \multicolumn{1}{l|}{55.33} &
   23.77 &
  48.44 \\ \hline
\multicolumn{1}{|l|}{Orienmask~\cite{Orienmask}} &
  \multicolumn{1}{l|}{ICCV21} &
  Darknet-53 &
  \multicolumn{1}{l|}{23.17} &
  \multicolumn{1}{l|}{28.96} &
  \multicolumn{1}{l|}{84.74} &
  \multicolumn{1}{l|}{63.58} &
  \multicolumn{1}{l|}{34.22} &
  \multicolumn{1}{l|}{54.12} &
  \multicolumn{1}{l|}{46.47} &
  31.78 & 45.88 \\ \hline
\multicolumn{1}{|l|}{QueryInst~\cite{QueryInst}} &
  \multicolumn{1}{l|}{ICCV21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{18.75} &
  \multicolumn{1}{l|}{27.95} &
  \multicolumn{1}{l|}{80.65} &
  \multicolumn{1}{l|}{82.41} &
  \multicolumn{1}{l|}{31.82} &
  \multicolumn{1}{l|}{47.62} &
  \multicolumn{1}{l|}{54.77} &
   20.41 &
   45.55 \\ \hline
\multicolumn{1}{|l|}{FASA~\cite{FASA}} &
  \multicolumn{1}{l|}{ICCV21} &
  ResNet-50-FPN &
  \multicolumn{1}{l|}{9.1} &
  \multicolumn{1}{l|}{19.58} &
  \multicolumn{1}{l|}{71.15} &
  \multicolumn{1}{l|}{63.18} &
  \multicolumn{1}{l|}{20.87} &
  \multicolumn{1}{l|}{34.70} &
  \multicolumn{1}{l|}{29.15} &
  12.28  & 32.50
   \\ 
   \hline
\tss (Ours) & & ResNet-50-FPN &
  \multicolumn{1}{l|}{\textbf{53.55}} &
  \multicolumn{1}{l|}{\textbf{46.94}} &
  \multicolumn{1}{l|}{\textbf{88.38}} &
  \multicolumn{1}{l|}{\textbf{80.71}} &
  \multicolumn{1}{l|}{\textbf{81.93}} &
  \multicolumn{1}{l|}{\textbf{79.96}} &
  \multicolumn{1}{l|}{\textbf{81.61}} &
  \multicolumn{1}{l|}{\textbf{67.24}} &
  \multicolumn{1}{l|}{\textbf{72.54}} 
  \\
  \hline
\end{tabular}%
}
\end{center}
	\caption{In \cref{tab:challenge_iou_without_post_processing} we have compared with \sota methods after fine-tuning them on EndoVis dataset. However, we propose a specific post-processing specially for the instrument segmentation scenario which does a non-maximal suppression across the classes. Such post-processing can be applied to other methods as well, and hence for a fair comparison we have done so. The table shows the results after post-processing. Note that other EndoVis methods already do a similar post-processing along with host of others. Hence their results do not change. Note that, we do not claim novelty/contribution over the suggested post-processing, as it is already implemented in EndoVis methods without formally describing/acknowledging it.}
	\label{tab:challenge_iou_after_post_processing}
\end{table*}

==> Tables/tab_comparison_CADIS.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllllll}
\hline
\textbf{Dataset} &
  \textbf{Method} &
  \textbf{Conference} &
  \textbf{Arch.} &
  \textbf{Ch\_ \iou} &
  \textbf{APm} &
  \textbf{ISI\_IOU} &
  \multicolumn{10}{l}{\textbf{Instrument Classes IOU}} &
  \textbf{mcIOU} \\ \cline{8-17}
\textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{C} &
  \textbf{CC} &
  \textbf{TF} &
  \textbf{PK} &
  \textbf{PH} &
  \textbf{LI} &
  \textbf{IH} &
  \textbf{SK} &
  \textbf{MM} &
  \textbf{CF} &
  \textbf{} \\ \hline
\multirow{23}{*}{\textbf{\cadis}} &
  \textbf{\nli Methods} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
 & CascadeRCNN                          & CVPR18    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & HTC                                  & CVPR19    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MaskScoring\_RCNN                    & CVPR19    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SipMask                              & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SimCal                               & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & CondInst                             & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & BMaskRCNN                            & ECCV20    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SOLO                                 & NeurIPS20 & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & SCNet                                & AAAI21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MFTA                                 & CVPR21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & DetectoRS                            & CVPR21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Orienmask                            & ICCV21    & Dknt53 &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & QueryInst                            & ICCV21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & FASA                                 & ICCV21    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Mask2Former                          & CVPR22    & Trfmr     &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-18} 
 & \textbf{\evs Methods} &           &           &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & TernausNet-11                        & ICMLA18   & UNet11    &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MF-TAPNET                            & MICCAI19  & UNet      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & MaskRCNN\_d                          & ICCV17    & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & ISINET                               & MICCAI20  & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & TraSeTR                              & ICRA22    & Trfmr     &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & S3NET (OURS)                         &           & R-50      &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}%
}
\caption{Performance of \sota instance segmentation methods on \cadis instrument segmentation dataset. APm represents Mean Average Precision of the mask, i.e., AP0.50:0.95}
\label{tab:comparison_CADIS_instance}
\end{table*}

==> Tables/tab_comparison_sota.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{lll}
\hline
     & \textbf{Model}  &  \textbf{APm} \\ \hline
 Two-stage & MaskRCNN~\cite{MaskRCNN}   & 45.7    \\  
& CascadeRCNN~\cite{CascadeRCNN}   & 39.6    \\  
     & MaskScoring\_RCNN~\cite{MaskScoringRCNN}   &  44.1    \\   
     & CondInst~\cite{CondInst} & 49.8           \\
     & BMaskRCNN~\cite{BMaskRCNN}    &    36.8      \\
Few-shot     & MFTA~\cite{MFTA} &  33.3      \\
Query-based    & QueryInst~\cite{QueryInst}   &   38.9      \\
 Two-stage + HTC   & HTC~\cite{HTC} &    45.2     \\
    & SCNet~\cite{SCNet}     &     43.9    \\
    & DetectoRS~\cite{DetectoRS}    & 52.5        \\
Long-tail specific & SimCal~\cite{SimCal}   &      42.3    \\
    & FASA~\cite{FASA}   &     29.7    \\
One-stage    & SOLO~\cite{SOLO} &   37.0       \\
     & Orienmask~\cite{Orienmask} &    43.5      \\
Video-Instance     & SipMask~\cite{SipMask} &  30.2         \\
EndoVis  & \tss (Ours) &  \textbf{58.2}          \\
     \hline
\end{tabular}%
}
\caption{Performance of \sota instance segmentation methods on EndoVis 2017 instrument segmentation dataset. APm represents Mean Average Precision of the mask, i.e., AP0.50:0.95}
\label{tab:comparison_sota}
\end{table}

==> Tables/tab_isinet_iou.tex <==
\begin{table*}[t]
\caption{Class-wise accuracy comparison with \sota (ISINet) on the metric proposed by them. We observe that our results are better for all classes of \evda including sparse class.}
\centering
\resizebox{\linewidth}{!}{ %
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
	\hline
	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{7}{c|}{Instrument Classes - \evda } & mean \\ \cline{3-9}
	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Vessel & Grasping & Monopolar & Ultrasound & class \\
	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Sealer & Retractor & Curved Scissors & Probe & IoU \\ \hline
	ISINet~\cite{gonzalez2020isinet} & 52.2 & 38.7 & 38.5 &	50.09 &	27.43 &	2.01&	28.72&	12.56&	28.96\\ \hline
	\tss (Ours) & \textbf{71.99} & \textbf{75.08} & \textbf{54.32} & \textbf{61.84} & \textbf{35.50} & \textbf{27.47} & \textbf{43.23} & \textbf{28.38} & \textbf{53.64} \\ \hline
\end{tabular}
}
\\ \vspace{1em}
\resizebox{\linewidth}{!}{ %
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}	
	\hline	
	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{7}{c|}{Instrument Classes- \evdb } & mean \\ \cline{3-9}
	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Monopolar & Ultrasound & Suction & Clip &  class\\
	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Curved Scissors & Probe & Instrument & Applier & IoU \\ \hline
	ISINet~\cite{gonzalez2020isinet} & 70.97 &  73.83 & 48.61 &	30.98 &	88.16 &	2.16&	37.68&	0.00 &	40.21\\ \hline
	\tss (Ours) & \textbf{74.02} & \textbf{77.22} & \textbf{50.87} & 19.83 & \textbf{92.12} & \textbf{7.44} & \textbf{50.59} & 0.00 & \textbf{42.58} \\ \hline
\end{tabular}
}
\\ \vspace{1em} %
\resizebox{\linewidth}{!}{ %
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}	
	\hline	
	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{10}{c|}{Instrument Classes- \eets } & mean \\ \cline{3-12}
	\multicolumn{1}{|c|}{} & ISINet & Suction & Irrigation & Spachula & Scissors & Knife & Navigation & Biopsy1 & Curette & Drill & Tumor &  class\\
	\multicolumn{1}{|c|}{} &IoU  &  &  &   &  &  &   & & & & Biopsy& IoU  \\ \hline
	ISINet~\cite{gonzalez2020isinet}& 46.23  & 77.26	& 35.44	& 1.18	& 0.00	& 3.67	& 41.59	& 14.45	& 23.98 & 4.21 &  7.66 & 20.94	 \\ \hline	
	\tss (Ours) & \textbf{49.19} & 76.36 & 29.95 & \textbf{9.15} & 0.00 & \textbf{7.22} & \textbf{46.44} & \textbf{30.46} & 9.82 & 0.00 & \textbf{44.91} & \textbf{25.43} \\ \hline
\end{tabular}%
}
\label{tab:ISINet_IoU}
\end{table*}

% \begin{table*}[t]
% \caption{Class-wise accuracy comparison our method with the best from \sota (ISINet). We report the results in terms of the metric proposed by ISINet itself, i.e., ISINet \iou, class-wise \iou, and mean class \iou. We observe that our results are better for all classes.}
% \centering
% \resizebox{\linewidth}{!}{ %
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
% 	\hline
% 	\multirow{3}{*}{{Method}} & \multicolumn{1}{l|}{} & \multicolumn{7}{c|}{Instrument Classes} & mean \\ \cline{3-9}
% 	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Vessel & Grasping & Monopolar & Ultrasound & class \\
% 	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Sealer & Retractor & Curved Scissors & Probe & IoU \\ \hline
% 	ISINet~\cite{gonzalez2020isinet}& 49.57 &	36.93&	37.8&	47.06&	24.96&	2.01&	19.99&	13.9&	26.92 \\ \hline	ISINet\_flow~\cite{gonzalez2020isinet} & 52.2 & 38.7 & 38.5 &	50.09 &	27.43 &	2.01&	28.72&	12.56&	28.96\\ \hline
% 	\tss (Ours) & \textbf{71.99} & \textbf{75.08} & \textbf{54.32} & \textbf{61.84} & \textbf{35.50} & \textbf{27.47} & \textbf{43.23} & \textbf{28.38} & \textbf{53.64} \\ \hline
% \end{tabular}
% }
% \\ \vspace{1em}
% \resizebox{\linewidth}{!}{ %
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}	
% 	\hline	
% 	\multicolumn{1}{|c|}{} & ISINet & Bipolar & Prograsp & Large & Monopolar & Ultrasound & Suction & Clip & mean class\\
% 	\multicolumn{1}{|c|}{} & IoU & Forceps & Forceps & Needle Driver & Curved Scissors & Probe & Instrument & Applier & IoU \\ \hline
% 	ISINet~\cite{gonzalez2020isinet}& 71.01 & 73.55 &	48.98&	30.38&  88.17&	 2.23&	37.84&	0.00 &	 40.16 \\ \hline	ISINet\_flow~\cite{gonzalez2020isinet} & 70.97 &  73.83 & 48.61 &	30.98 &	88.16 &	2.16&	37.68&	0.00 &	40.21\\ \hline
% 	\tss (Ours) & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \hline
% \end{tabular}
% }
% \\ \vspace{1em} %
% \resizebox{\linewidth}{!}{ %
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}	
% 	\hline	
% 	\multicolumn{1}{|c|}{} & ISINet & Suction & Irrigation & Spachula & Scissors & Knife & Navigation & Biopsy1 & Curette & Drill & Tumor & mean class\\
% 	\multicolumn{1}{|c|}{} &IoU  &  &  &   &  &  &   & & & & Biopsy& IoU  \\ \hline
% 	ISINet~\cite{gonzalez2020isinet}& 46.23  & 77.26	& 35.44	& 1.18	& 0.00	& 3.67	& 41.59	& 14.45	& 23.98 & 4.21 &  7.66 & 20.94	 \\ \hline	ISINet\_flow~\cite{gonzalez2020isinet} &  &  &  &	 &	 &	&	& & & &	&	\\ \hline
% 	\tss (Ours) & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \hline
% \end{tabular}%
% }
% \label{tab:ISINet_IoU}
% \end{table*}

==> Tables/tab_miou_CADIS.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
\hline
~\textbf{Instrument} & ~\textbf{UPerNet} & ~\textbf{HRNetV2} & ~\textbf{TraSeTR} & ~\textbf{\tss}  \\
~\textbf{classes}            &  ~\cite{upernet}       &  ~\cite{hrnetv2}      &   ~\cite{TraSeTR}      & ~\textbf{(Ours)} \\ \hline
Cannula            & 50      & 49.5    & 53.1    &        \\
Cap. Cystotome     & 54.5    & 61.7    & 64.4    &        \\
Tissue Forceps     & 74      & 78      & 79.2    &        \\
Primary Knife      & 89.5    & 89.3    & 92.3    &        \\
Ph. Handpiece      & 77.6    & 77.9    & 76.2    &        \\
Lens Injector      & 81      & 82.8    & 87.1    &        \\
I/A Handpiece      & 73.6    & 75.3    & 71.3    &        \\
Secondary Knife    & 68.2    & 79.5    & 82.7    &        \\
Micromanipulator   & 63.6    & 64.4    & 66.3    &        \\
Cap. Forceps       & 23      & 27.2    & 26.1    &        \\ \hline
Total              & 65.5    & 68.6    & 69.9    &        \\ \hline
\end{tabular}%
}
\caption{Segmentation results on \cadis dataset.}
\label{tab:comparison_CADIS_miou}
\end{table}

==> src_main/P_Dataset_And_Evaluation.tex <==
\section{Dataset and Evaluation}

\myfirstpara{Benchmark Datasets}
%
We have used Robot-assisted endoscopic surgery datasets EndoVis 2017~\cite{EndoVis_2017} (denoted as \evda), and  EndoVis 2018~\cite{EndoVis_2018} (denoted as \evdb) 
%and microscopic cataract surgery (\cadis)~\cite{cadis} 
datasets for our experiments.
\begin{enumerate*}[label=\textbf{(\arabic*)}]
% 
\item \evda dataset contains ten videos from the da-Vinci robotic system and provides annotations of 6 robotic instruments and an ultrasound probe. We adopted the 4-fold cross-validation from \cite{TernausNet} for fair comparison with 1800 frames ($8 \times 225$). The fold-wise split makes it 1350 and 450 frames for training and validation, respectively.
%
\item \evdb is a robotic instrument clinical dataset that includes organs and surgical items like gauze and suturing thread and contains the instrument super category but not the instrument type. This dataset is additionally annotated for instrument types by \cite{gonzalez2020isinet} with seven robotic instrument types and 11 training videos, and four testing videos with 149 images each. They provide the annotations as image pixels but do not provide instance labels. We annotated the instances ourselves for our experiments.
% \footnote{We note that there are other datasets for medical image segmentation released as part of the EndoVis Challenge \cite{RobustMIS2019,grammatikopoulou2019cadis,HeiSurF_dataset}. Similar to \evdb, they also do not contain either class type or instance labels. While we annotated \evdb ourselves, we did not extend this to other datasets due to the large amount of effort involved.}.
%\item \cadis dataset, is a microscopic cataract surgery dataset with 25 videos with semantic segmentation of the scene. The instance segmentation of 10 instrument types were generated as in ~\cref{tab:comparison_CADIS_miou} from the images and we adopted the train-test split as mentioned in~\cite{cadis, TraSeTR} for our experiments.
\end{enumerate*}

\mypara{Evaluation}
%
We categorize the compared methods into two categories. \evs methods are the ones that have reported their accuracy on \evda or \evdb datasets. \nli models are the instance segmentation methods proposed for natural images. For \evda and \evdb datasets, we evaluate the performance on the Challenge \iou (Ch\_\iou) metric as proposed in the \evda challenge~\cite{allan20192017} and ISINet \iou (ISI\_\iou) and mean class \iou (mc\iou) metrics proposed in~\cite{gonzalez2020isinet}. 
%For \cadis dataset, we use mean Intersection over Union (mIoU) (m\iou) as mentioned in the~\cite{cadis} for the 10 selected instrument classes.

% \mypara{Proposed Dataset (\eets)}
% %
% %\input{Images/fig_eets}
% \eets is the proposed clinical neurosurgery dataset with 10 instrument types, and 20 videos for training, and 10 videos for testing. Each video is of 5 seconds, and contains 125 frames, from clinical EETS neurosurgery performed on nine different patients by an expert neurosurgeon.
 
%RobustMIS2019~\cite{RobustMIS2019} provides instance segmentation without class type annotations. CADIS2020~\cite{grammatikopoulou2019cadis} introduces a dataset for the semantic segmentation of cataract surgery videos without instance labels. HeiSurF2021~\cite{HeiSurF_dataset} is a dataset for work flow analysis and full scene segmentation without instances. Hence, these datasets are not included in our study.
% of fine-grained instance segmentation of surgical instruments. %We use only the type segmentation annotations for our experiments.

% For \evda, we train our model for 4 folds, with 1350 frames (6 videos) used for training and 450 frames (2 videos) used for testing in each iteration. In each fold, we generate predictions for 2 videos, which are collected for all the 8 videos, during the cross-validation \cite{TernausNet}. For obtaining the results of challenge \iou, the results for all 8 videos are then analyzed together to handle the scenario where a set of classes are not present in one of the validation splits. This metric is commonly used and it consider only the classes presented in a given frame for evaluation. 

% The instrument segmentation of robotic surgical scenes was first introduced in EndoVis2015 ~\cite{endovis_2015}. The objective was extracting the instrument from background or binary segmentation and segmentation of the instrument parts. There was no instrument type or instance segmentation available. EndoVis2017 dataset is a robotic instrument simulation dataset containing annotations for instrument parts and different instrument types. EndoVis2018 is a robotic instrument real surgical dataset that includes organs and surgical items like gauze and suturing thread and contain the instrument super category but not the instrument type. This dataset is additionally annotated for instrument types by ~\cite{gonzalez2020isinet} but they provide the annotations as image pixels and does not contain instance affiliation of the pixels. 

% RobustMIS2019~\cite{RobustMIS2019} provides instance segmentation without class type annotations. CADIS2020~\cite{grammatikopoulou2019cadis} introduces a dataset for the semantic segmentation of cataract surgery videos without instance affiliation. HeiSurF2021~\cite{} is a dataset for work flow analysis and full scene segmentation. Sinus-Surgery
% dataset of~\cite{qin2020towards} includes the binary annotation of instruments. Hence, these datasets are not applicable for the fine-grained instance segmentation of surgical instruments.


% In the \evs category, for \cite{TernausNet} and \cite{gonzalez2020isinet}, we use the four pre-trained EndoVis models corresponding to each fold provided by the authors. For MF\_TAPNet~\cite{MFTAPNet} we train their supervised setup on the TAPNet model with default parameters to obtain four models. 
% For \nli methods, we train their network for the \evda dataset with default parameters. 
% in \cref{tab:comparison_sota}, and ISINet on their proposed metric in \cref{tab:ISINet_IoU}. 
%train all the methods with the train set and report the results on test set. The challenge \iou results are shown in \cref{tab:challenge_iou_without_post_processing} and generalization of our method on all datasets is evident with results as it out performs the \sota methods for all the different datasets.


